Multi-Agent Contract Design: How to Commission Multiple Agents with Individual Outcome

We study hidden-action principal-agent problems with multiple agents. These are problems in which a principal commits to an outcome-dependent payment scheme in order to incentivize some agents to take costly, unobservable actions that lead to favorable outcomes. Previous works on multi-agent problems study models where the principal observes a single outcome determined by the actions of all the agents. Such models considerably limit the contracting power of the principal, since payments can only depend on the joint result of all the agents' actions, and there is no way of paying each agent for their individual result. In this paper, we consider a model in which each agent determines their own individual outcome as an effect of their action only, the principal observes all the individual outcomes separately, and they perceive a reward that jointly depends on all these outcomes. This considerably enhances the principal's contracting capabilities, by allowing them to pay each agent on the basis of their individual result. We analyze the computational complexity of finding principal-optimal contracts, revolving around two newly-introduced properties of principal's rewards, which we call IR-supermodularity and DR-submodularity. Intuitively, the former captures settings with increasing returns, where the rewards grow faster as the agents' effort increases, while the latter models the case of diminishing returns, in which rewards grow slower instead. These two properties naturally model two common real-world phenomena, namely diseconomies and economies of scale. In this paper, we first address basic instances in which the principal knows everything about the agents, and, then, more general Bayesian instances where each agent has their own private type determining their features, such as action costs and how actions stochastically determine individual outcomes.

==> src/Envelope.tex <==
\section{newnew proof}
Let $L(z,\lambda)=\max\limits_{i \in N,\phi \in \Phi^i} \left( U^i \phi^i z- \lambda C \phi^i z - U^i z\right)$,

Clearly if $L(z,\lambda)=0$, then $z$ is an equilibrium.

We need to show that for each local minimum of the bi-convex problem it holds $L(z,\lambda)=0$.
Formally, $\bar z, \bar \lambda$ is a local minimum if:
\begin{itemize}
	\item $\min_\lambda L(\bar z,\lambda)= L(\bar z,\bar \lambda)$
	\item $\min_z L( z,\bar \lambda)= L(\bar z,\bar \lambda)$
\end{itemize}


Let $L(z,\lambda,i,\phi^i)= \left( U^i \phi^i z- \lambda C \phi^i z - U^i z\right)$
\begin{lemma}
	if $(z,\lambda)$ is a local optimum, there exists a $i(z,\lambda),\phi(z,\lambda)\in \argmax_{i \in N,\phi \in  \Phi^i} \sum_i\left( U^i \phi^i z- \lambda_i C \phi^i z - U^i z\right)$ 
	such that $\lambda=\argmin_{\lambda'} L(z,\lambda',i(z,\lambda),\phi(z,\lambda))$ and $z=\argmin_{z'} L(z',\lambda,i(z,\lambda),\phi(z,\lambda))$
\end{lemma}

Hence, $ \lambda C \phi^{i(z,\lambda}(z,\lambda) z =0$ and $  C \phi(z,\lambda) z\le 0$  by the Optimality of $\lambda$. \ma{si dimostrano facili con le KKT e Daskin}

By the optimality of z, we have that since $\phi(z,\lambda) z$ is safe for agent $i(z,\lambda)$,
\begin{align}
&\left( U^{i(z,\lambda)} \phi(z,\lambda) z- \lambda C \phi(z,\lambda) z - U^{i(z,\lambda)}  z\right) \\
&\le  \left( U^{i(z,\lambda)} \phi(z,\lambda)\phi(z,\lambda) z- \lambda C \phi(z,\lambda) \phi(z,\lambda) z - U^{i(z,\lambda)} \phi(z,\lambda) z\right)  \\
&=  \left( U^{i(z,\lambda)} \phi(z,\lambda)\phi(z,\lambda) z- \lambda C \phi(z,\lambda) \phi(z,\lambda) z - U^{i(z,\lambda)} \phi(z,\lambda) z + \lambda C  \phi(z,\lambda) z  \right) \le 0
\end{align}
where the last inequality comes from the optimality of the deviation $ \phi(z,\lambda)$.

\section{a Polynomial-time Algorithm}

\mat{non funziona un cazzo. Con gli approximate local minima non riesco a dimostrare che è un epsilon equilibrium. il problema è che $i^*, \phi^*$ non è un subgradiente per $z^*$.}


Extend $L$ with a $\delta$-strongly convex function on $z$.
Run alternate convex optimization until we find an 

$\lambda^*\in \argmin_{\lambda} L( z^*,\lambda) $
and $z^*$ such  that $L(z^*)\le \argmin_{z} L( z,\lambda^*)+\epsilon$.


By the optimality of $\lambda^*$ we have that there exists a $i^*$ and $\phi^*$ such that $ \lambda^* C \phi^* z^* =0$ and $C \phi^* z^*\le 0$.(KKT)

Let $\bar z$ be the optimal z and $i',\phi'$ the optimal deviation in $\bar z$ that satisfies the KKT.

Then, 

\begin{align}
L(z^*,\lambda^*)& \le  \left( U^{i'} \phi' \bar z- \lambda C \phi'  \bar z - U^{i'}  \bar z\right)  +\epsilon \\
& \le \left( U^{i'} \phi' \bar z- \lambda C \phi' z^* - U^{i'}  \bar z\right)  \\
&\le 
&\le \left( U^{i'} \phi^*  z^*- \lambda C \phi^*   z^* - U^{i'}  \bar z\right) + \epsilon\\
& \le \left( U^{i'} \phi^*  z^*-  U^{i'}  \bar z\right) + \epsilon\\
& \le \left( U^{i'} \phi^*  z^*-  U^{i'}  \bar z\right) + \epsilon
\end{align}


\begin{align}
L(z^*,\lambda^*)&\le L(\bar z,\lambda^*) +\epsilon\\
&=\max_{i,\phi}\left( U^{i}  \phi \bar z- \lambda C  \phi \bar z - U^{i} \phi \bar z\right) \\
&\le  \left( U^{i^*}  \phi^* \bar z- \lambda C  \phi^* \bar z - U^{i^*}  \bar z\right)   + \epsilon+ \delta \\
&=  \left( U^{i(z,\lambda)} \phi(z,\lambda)\phi(z,\lambda) z- \lambda C \phi(z,\lambda) \phi(z,\lambda) z - U^{i(z,\lambda)} \phi(z,\lambda) z + \lambda C  \phi(z,\lambda) z  \right) \le 0
\end{align}


%\section{new Proof}
%
%Let $L(z,\lambda)=\max\limits_{\phi \in \bar \Phi} \sum_i\left( U^i \phi^i z- \lambda C \phi^i z - U^i z\right)$,
%where $\bar \Phi$ is the set of deviation in which at most 1 deviation is different from the identity matrix.
%
%Clearly if $L(z,\lambda)=\max\limits_{\phi \in \bar \Phi} \sum_i\left( U^i \phi^i z- \lambda_i C \phi^i z - U^i z\right)=0$, then $z$ is an equilibrium.
%
%We need to show that for each local minimum of the bi-convex problem it holds $L(z,\lambda)=0$.
%Formally, $\bar z, \bar \lambda$ is a local minimum if:
%\begin{itemize}
%	\item $\min_\lambda L(\bar z,\lambda)= L(\bar z,\bar \lambda)$
%	\item $\min_z L( z,\bar \lambda)= L(\bar z,\bar \lambda)$
%\end{itemize}
%
%Let $L(z,\lambda,\phi)= \sum_i\left( U^i \phi^i z- \lambda C \phi^i z - U^i z\right)$
%\begin{lemma}
%if $(z,\lambda)$ is a local optimum, there exists a $\phi(z,\lambda)\in \argmax_{\phi \in \bar \Phi} \sum_i\left( U^i \phi^i z- \lambda_i C \phi^i z - U^i z\right)$ 
%such that $\lambda=\argmin_{\lambda'} L(z,\lambda',\phi(z,\lambda))$ and $z=\argmin_{z'} L(z',\lambda,\phi(z,\lambda))$
%\end{lemma}
%
%Hence, $\sum_i \lambda C \phi^i(z,\lambda) z =0$ and $\sum_i  C \phi^i(z,\lambda) z\le 0$  by the Optimality of $\lambda$. 
%%%The second one implies that $C \phi^i(z,\lambda) z=0$ for each $i$.
%
%Hence, for each constraint c we have two possibilities: 
%\begin{itemize}
%	\item  $\sum_i \lambda_c C_c \phi^i(z,\lambda) z = 0$, implying  
%	\item $\sum_i \lambda_c C_c \phi^i(z,\lambda) z <0$ and $\lambda_i=0$. 
%\end{itemize}
%Now, let $i^*$ be the only agent such that $\phi^{i^*}(z,\lambda)\neq I$.
%
%By the optimality of z, we have that since $\phi(z,\lambda) z$ is safe it holds
%\begin{align}
% &\sum_i\left( U^i \phi^i(z,\lambda) z- \lambda_i C \phi^i(z,\lambda) z - U^i z\right) \\
% &\le  \sum_i\left( U^i \phi^i(z,\lambda)  \phi^{i^*}(z,\lambda) z- \lambda_i C \phi^i(z,\lambda)  \phi^{i^*}(z,\lambda) z - U^i  \phi^{i^*}(z,\lambda)z\right) \\
% &\le \sum_{i \neq i^*} \left( U^i  \phi^{i^*}(z,\lambda) z- \lambda_i C  \phi^{i^*}(z,\lambda) z - U^i \phi^{i^*}(z,\lambda) z\right)  +  \left( U^{i^*} \phi^{i^*}(z,\lambda) \phi^{i^*}(z,\lambda)  z- \lambda_{i^*} C \phi^{i^*}(z,\lambda) \phi^{i^*}(z,\lambda) z - U^{i^*} \phi^{i^*}(z,\lambda) z\right)\\
% &\le 0+\left( U^{i^*} \phi^{i^*}(z,\lambda) \phi^{i^*}(z,\lambda) z- \lambda_{i^*} C \phi^{i^*}(z,\lambda) \phi^{i^*}(z,\lambda)  z - U^{i^*} \phi^{i^*}(z,\lambda) z\right)\le 0 ,
% \end{align}
%where the last inequality comes from the optimality of the deviation $ \phi^{i^*}(z,\lambda)$.

==> src/Introduction.tex <==
\section{Introduction}


Over the last years, equilibrium computation problems have received a terrific attention from AI and ML research~\citep{brown2019superhuman,meta2022human}, as game-theoretical equilibrium notions provide a principled framework to deal with multi-player decision-making problems.
%
Most of the works on equilibrium computation problems focus on classical solution concepts---such as the well-known \emph{Nash equilibrium} (NE)~\citep{nash1951non} and \emph{correlated equilibrium} (CE)~\citep{aumann1974subjectivity}---, thus neglecting the presence of constraints entirely.
%
However, in most of the real-world applications, the players are usually subject to constraints that rule out the feasibility of some of their strategies, such as, \emph{e.g.}, safety requirements and budget caps.
%
%
%However, the most widely studied notions of equilibrium---such as the well-known \emph{Nash equilibrium} (NE)~\citep{nash1951non} and \emph{correlated equilibrium} (CE)~\citep{aumann1974subjectivity}---entirely neglect the presence of constraints. 
%
Thus, addressing equilibrium notions involving constraints is a crucial step needed for the operationalization of game-theoretic concepts into real-world settings.



The study of equilibrium notions involving constraints was initiated by~\citet{arrow1954existence}, who define the concept of \emph{generalized} NE (GNE).
%
The GNE can be interpreted as an NE of a game where players' strategies are subject to some constraints, which must be satisfied at the equilibrium and also determine which are the feasible players' deviations.
%
% The computational study of GNEs has been initiated by~\citet{rosen1965existence}, and~\citep{kanzow2016augmented,bueno2019optimality,jordan2022first} are some of the most recent works on the topic (see~\citep{facchinei2010generalized} for a survey of earlier works).
%
% and, since then, many works addressed the problem of computing GNEs by mainly exploiting techniques based on \emph{quasi-variational inequalities} (see~\citep{facchinei2010generalized} for a survey).
%
However, given that computing a GNE is clearly $\mathsf{PPAD}$-hard~\citep{daskalakis2009complexity}, all the works dealing with the computation of GNEs (see, \emph{e.g.},~\citep{facchinei2010generalized}) provide efficient algorithms only in specific settings that require very stringent assumptions. 
%
% More recently, some works~\citep{kanzow2016augmented,bueno2019optimality,jordan2022first} also studied the convergence of learning dynamics  


Most of the computationally challenges in finding GNEs are inherited from the NE.
%
In settings in which constrained are \emph{not} involved, the computational issues of NEs are usually circumvented by considering weaker equilibrium notions.
%
Among them, those that have received most of the attention in the literature are the CE and its variations, which have been shown to be efficiently computable in several settings of interest~\citep{papadimitriou2008computing,celli2020no}.
%
Surprisingly, with the only exception of~\citep{chenfinding} (see Section~\ref{sec:related} for a detailed discussion on it), no work has considered the problem of computing CEs in constrained settings.
%
Thus, investigating whether the CE retains its nice computational properties when adding constraints on players' strategies is an open interesting question.




\subsection{Original Contributions}


In this paper, we introduce and computationally characterize \emph{constrained Phi-equilibria}, starting, as it is customary, from the setting of \emph{normal-form games}.
%
Our equilibria include the constrained versions of the classical CE and all of its variations as special cases, by generalizing the notion of Phi-equilibria introduced by~\citet{greenwald2003general} to constrained settings.
%
In particular, constrained Phi-equilibria are defined as Phi-equilibria, but in games where players are subject to some constraints.
%
Such constraints must be satisfied at the equilibrium, and, additionally, players are only allowed to undertake \emph{safe deviations}, namely those that are feasible according to the constraints.
%
%by players' deviations in order for them to be safe (\emph{i.e.}, feasible according to the constraints).
%
Crucially, the set of safe deviations of a player does \emph{not} only depend on the strategy of that player, but also on those of the others.


We start by showing that one of the most appealing computational properties of Phi-equilibria, namely that the set of the equilibria of a game is convex, is lost when moving to their constrained version.
%
This raises considerable computational challenges in computing constrained Phi-equilibria.
%
Indeed, we formally prove a strong intractability result: for any factor $\alpha > 0$, it is \emph{not} possible, unless $\mathsf{P} = \mathsf{NP}$, to find in polynomial time a constrained (approximate) Phi-equilibrium which achieves a multiplicative approximation $\alpha$ of the optimal value of a given linear function.
%
Then, in the rest of the paper, we show several ways in which such a negative result can be circumvented.



We prove that a constrained approximate Phi-equilibrium which maximizes a given linear function can be found in polynomial time, when either the number of constraints or that of players' actions is fixed.
%
Our results are based on a general algorithm that employs a non-standard ``Lagrangification'' of the constraints defining the set of safe deviations of a player.
%, and a clever discretization 
%
Moreover, the algorithm needs a way of dealing with the non-convexity of the set of the equilibria, which we provide in the form of a clever discretization of the space of the Lagrange multipliers.



Finally, we focus on the special case in which the constraints defining the safe deviations of a player do \emph{not} depend on the the strategies of the other players, but only on the strategy of that player.
%
This includes constrained Phi-equilibria identifying a particular constrained version of the \emph{coarse} CE by~\citet{moulin1978}, in which the players' strategies are subject to \emph{marginal cost constraints}.
%
These arise in several real-world applications in which the players have bounded resources, such as, \emph{e.g.}, budget-constrained bidding in auctions.
%
In such a special case, we prove that a constrained (exact) Phi-equilibrium maximizing a given linear function can be computed in polynomial time, and we provide an efficient decentralized no-regret learning algorithm for finding \emph{one} constrained (approximate) Phi-equilibrium.


%We conclude the paper by introducing a challenging open question related to the problem studied in this paper, paving the way for future research on the topic.


 


\subsection{Related Works}\label{sec:related}

%Next, we survey the works that are the most related to ours.

\paragraph{GNEs}
%
\citet{rosen1965existence} initiated the study of the computational properties of GNEs.
%
% introduced by~\cite{arrow1954existence} to study the equilibria of abstract economies. GNE can be seen as a generalization of Nash equilibria in constrained games in which both player's strategies and best responses are constrained to satisfy some costs constraints.
%
After that, several other works addressed the problem of computing GNEs by mainly exploiting techniques based on \emph{quasi-variational inequalities} (see~\citep{facchinei2010generalized} for a survey).
%
%several other works deepened the understanding of GNE in games, see~\citet{facchinei2010generalized} for a survey on the earlier works, mainly based on \emph{quasi-variational inequalities}.
%
More recently, some works~\citep{kanzow2016augmented,bueno2019optimality,jordan2022first,goktasexploitability} also studied the convergence of iterative optimization algorithms to GNEs.
%
%More recently the following works~\cite{kanzow2016augmented, bueno2019optimality, jordan2022first} addressed the convergence guarantees of learning GNE with the common assumption of the constrain space being jointly convex.
%
In order to provide efficient algorithms, all these works need to introduce very stringent assumptions, which are even stronger than those required for the efficient computation of NEs.


\paragraph{Constrained Markov Games}
%
Equilibrium notions involving constraints have also been addressed in the literature on \emph{Markov games}, with~\citep{altman2000constrained, alvarez2006existence} being the first works introducing GNEs in such a field.
%
More recently, \citet{hakami2015learning} defined a notion of constrained CE in Markov games.
%
However, the incentive constraints in their notion of equilibrium only predicate on ``pure'' deviations, which, in presence of constraints, may lead to empty sets of safe deviations.
%
Very recently,~\citet{chenfinding} generalize the work of~\citet{hakami2015learning} by considering ``mixed'' deviations.
%
However, their algorithm provides rather weak convergence guarantees, as it only ensures that the returned solution satisfies incentive constraints in expectation.
%
Indeed, as we show in Proposition~\ref{prop:non-convex}, the set of constrained equilibria may \emph{not} be convex (it is easy to see that Example~\ref{example} also applies to the setting studied by~\citet{chenfinding}), and, thus, the fact that incentive constraints are only satisfied in expectation does \emph{not} necessarily imply that the ``true'' incentive constraints defining the equilibrium are satisfied.
%
We refer the reader to Appendix~\ref{app:weakness} for additional details on these aspects.
%
%
%
%Concurrently, constrained Nash equilibria where studied in the Safe Reinforcement Learning community, starting from~\citet{altman2000constrained, alvarez2006existence} these work introduces the concept of GNE in the field of Markov Games.
%More recently, the study of equilibria in Markov Games was extended to the concept of Correlated Equilibria~\citep{aumann1974subjectivity} defining Constrained Markov Games~\citep{hakami2015learning,chenfinding}. Specifically~\citet{chenfinding} is the only work that considers solution concepts other the Nash in Constrained Markov Games. However, their algorithm only finds a relaxed solution concept, which satisfies the correlated equilibria incentives only in expectation.


%
%Anther line of work connected to this paper is the one that studies Phi-equilibria. This line of study was introduced by~\citet{greenwald2003general} and~\citet{stoltz2007learning}. They generalize the concept of Correlated Equilibria and unify many other solution concepts, such as Coerced Correlated Equilibria.



==> src/KKT.tex <==
\section{Correlated with KKT}

Define $V(z):=\max\limits_\phi\psi(z,\phi)$, where $\psi(z,\phi)=\sum\limits_{i}(U^i\phi^i-U^i)z$. 
%Then write the KKT for the optimization problem $\min\limits_{z\in\Delta} V(z)$: 
%
%\[
%	\begin{cases}
%		0\in\partial V(z)-\lambda+\nu 1\\
%		z_i\ge 0\\
%		\lambda_i\ge 0\\
%		\lambda_i z_i = 0\\
%		z^\top 1 = 1
%		
%	\end{cases}
%\]
%
%And by daskin's theorem we have that:
%\[
%\partial V(z) = \text{co}\left\{\sum\limits_{i} \left(U^i\phi^i-U^i\right)\Big\vert \phi\in BR(z)\right\}
%\]
%
%where $BR(z):=\argmax\limits_{\phi\in\Phi}\psi(z,\phi)$ and it is a convex polytope.
%Thus there exists a $\tilde\phi\in\text{co} BR(z)=BR(z)$ s.t. $\partial V(z)\ni\nabla_z\psi(z,\tilde\phi) = \lambda - \nu 1$ and $z,\lambda, \nu$ are variable which satisfy the KKT system.



The dual problem reads of $\min\limits_{z\in\Delta} V(z)$ reads $\sup\limits_{\lambda\ge0, \nu\in\Reals}g(\lambda,\nu)$ where: 

\[
g(\lambda,\nu) = 
%\inf\limits_{z\in \Reals^n} \left\{V(z)-\lambda^\top z+\nu(z^\top 1-1)\right\}=
-\nu + \inf\limits_{z\in \Reals^n} \left\{V(z)-\lambda^\top z+\nu z^\top 1\right\}=
	\begin{cases}
		-\nu+\inf\limits_{z\in\Reals^n}V(z)&\text{if}\quad \lambda =\nu 1\\
		-\infty&\text{otherwise}
	\end{cases}
\]

And thus the optimal value for the dual problem is attained at $\nu=0$ and $\inf\limits_{z\in\Reals^n}V(z)=0$. 
%This follows from the fact that $V(z)$ it is convex and unconstrained and thus in the optimal $z$ we have $0=\nabla_z\psi(z,\tilde\phi)=\sum\limits_{i}(U^i\tilde\phi^i-U^i)\in\partial V(z)$ for a certain $\tilde\phi\in BR(z)$ and thus $V(z)=0$ since $V(z) = \psi(z,\tilde\phi)=\nabla_z\psi(z,\tilde\phi)^\top z$. 
The fact that $\inf_zV(z)=0$ follows from the fact that $V(z)\ge0$ and $V(0)=0$.

Thus the value is $0$ also for the primal problem, since it is convex we have $0$ duality gap.

==> src/Optimal.tex <==
\section{Computing Optimal Constrained $\epsilon$-Phi-equilibria Efficiently}\label{sec:optimal}


In this section, we show how to circumvent the negative result established by Theorem~\ref{thm:hardness}.
%
In particular, we prove that, when the number of cost constraints is fixed, problem \textsc{ApxCPE}$(1,\epsilon)$ can be solved in time polynomial in the instance size and $\frac{1}{\epsilon}$ for $\epsilon > 0$ (Corollary~\ref{cor:res_1}).
%
Moreover, we also prove that, in general, for any constant $\epsilon > 0$ problem \textsc{ApxCPE}$(1,\epsilon)$ admits a quasi-polynomial-time algorithm, whose running time becomes polynomial when the number of players' actions is fixed (Corollary~\ref{cor:res_2}).
%
%, whenever the number of players and that of actions are fixed, the same problem admits a quasi-polynomial-time algorithm (Corollary~\ref{cor:res_2}).


First, in Section~\ref{sec:optimal_1}, we provide a general algorithm that is at the core of the two main results of this section.
%
Then, in Section~\ref{sec:optimal_1}, we show how the algorithm can be suitably instantiated in order to prove each result.
%
In the rest of this section, unless stated otherwise, we always assume that an $\epsilon > 0$ has been fixed, and that $I := (\Gamma,\Phi)$ and $\ell : \Delta_{\A} \to \mathbb{R}$ are the inputs of a given instance of problem \textsc{ApxCPE}$(1,\epsilon)$.


\subsection{General Algorithm}\label{sec:optimal_1}


The main technical tool that we employ in order to design our algorithm is a ``Lagrangification'' of the constraints defining the sets $\Phi_i^{\mcS}(\zvec)$ of safe deviations.
%
% By means of duality arguments, this allows us to reduce our problem to that of finding optimal Phi-equilibria in games without cost constraints.
%
%\ma{recap iniziale}
%\ma{dire che fissiamo un Phi qualsiasi che soddisfa ass 1}
%In this section, we show that whenever Assumption~\ref{ass:strictly} is satisfied and the number of constraints is contant, the problem  ???-$(\ell,1,\epsilon)$ can be solved in polynomial-time in the instance size and $\frac{1}{\epsilon}$. anche QPTAS/PTAS quando num actions constante.
%
%As a first step, we show that it is possible to Lagrangify and linearize the constraint regarding the safety of the violations. Formally, we prove the following.
%
%
First, we prove the following preliminary result, which shows that strong duality holds for the problem $\max_{\phi_i \in \Phi_i^\mcS(\zvec)} u_i(\phi_i \diamond \zvec)$ of finding the best safe deviation for player $i \in \N$ at $\zvec \in \Delta_{\A}$.
%
%
\begin{restatable}{lemma}{minmax}\label{lem:minmax}
	For every $\zvec\in \Delta_{\A}$ and $i \in \N$, it holds 
	\begin{align*}
		\max_{\phi_i \in \Phi_i^\mcS(\zvec)} u_i(\phi_i \diamond \zvec)& =\sup\limits_{\phi_i\in\Phi_i} \inf_{\etavec_i \in \mathbb{R}^{m}_+}  \left(u_i(\phi_i\diamond \zvec)-\etavec_i^{\top} \cvec_i(\phi_i \diamond \zvec)\right) \\
		& =\inf_{\etavec_i \in \mathbb{R}^{m}_+}  \sup\limits_{\phi_i\in\Phi_i} \left(u_i(\phi_i \diamond\zvec)-\etavec_i^{\top} \cvec_i(\phi_i \diamond\zvec)\right).
	\end{align*}
\end{restatable}
%
Then, by exploiting Lemma~\ref{lem:minmax}, we can prove that, under Assumption~\ref{ass:strictly}, strong duality continues to hold even when restricting the Lagrange multipliers $\etavec_i $ to have $\ell_1$-norm less than or equal to $1/\rho$.
%
%Let $V_{z,i}=\min_{\eta_i \in \mathbb{R}_+^?} \max\limits_{\phi^i}\left(U^i(\phi^i z)-\eta^i C(\phi^i z)\right)= \max\limits_{\phi^i} \min_{\eta_i \in \mathbb{R}_+^?} \left(U^i(\phi^i z)-\eta^i C(\phi^i z)\right)  $
%
Formally:
%
\begin{restatable}{lemma}{duality}\label{lem:duality}
	Let $\D\coloneqq \left\{\etavec\in\Reals^{m}_+ \mid  ||\etavec||_1\le{1}/{\rho}\right\}$.
	%
	Then, for every $\zvec\in \Delta_{\A}$ and $i \in \N$, it holds:
	\begin{align*}
	\max_{\phi_i \in \Phi_i^{\mcS}(\zvec)} u_i(\phi_i \diamond \zvec)	& =  \max\limits_{\phi_i\in\Phi_i} \min_{\etavec_i \in  \D} \left(u_i(\phi_i \diamond \zvec)-\etavec_i^\top \cvec_i(\phi_i\diamond \zvec)\right) \\
	&=\min_{\etavec_i \in \D} 	\max\limits_{\phi_i\in\Phi_i}\left(u_i(\phi_i \diamond \zvec)-\etavec_{i}^\top \cvec_i(\phi_i \diamond \zvec)\right) .
	 \end{align*}
\end{restatable}
%
Lemma~\ref{lem:duality} allows us to write player $i$'s incentive constraints in the definition of constrained $\epsilon$-Phi-equilibria as
\begin{equation}\label{eq:cons_lemmiz}
	u_i(\zvec) \geq \min_{\etavec_i \in \D} 	\max_{\phi_i\in\Phi_i}\left(u_i(\phi_i \diamond \zvec)-\etavec_{i}^\top \hspace{-0.1mm} \cvec_i(\phi_i \diamond \zvec)\right) - \epsilon.
\end{equation}
%
% $u_i(\zvec) \geq \min_{\etavec_i \in \D} 	\max_{\phi_i\in\Phi_i}\left(u_i(\phi_i \diamond \zvec)-\etavec_{i}^\top \cvec_i(\phi_i \diamond \zvec)\right) - \epsilon$.


This crucially allows us to show the following result: solving problem \textsc{ApxCPE}$(1,\epsilon)$ is equivalent to computing $\max_{(\etavec_1,\ldots,\etavec_n)\in\D^n} F_{\epsilon} (\etavec_1, \ldots, \etavec_{n})$, where $F_{\epsilon} (\etavec_1, \ldots, \etavec_{n})$ is the optimal value of a suitable maximization problem parameterized by tuples of Lagrange multipliers $\etavec_i \in \D$, one per player $i \in \N$.
%
% In order to do so, we first introduce a maximization problem parameterized by a tuple of Lagrange multipliers $\etavec_i \in \mathbb{R}_+^m$, one for each player $i \in \N$.
%
Such a problem
%, which we call $F_{\ell,\epsilon}(\etavec_1, \ldots, \etavec_{n})$, 
asks to compute a safe correlated strategy maximizing the linear function $\ell$ subject to players' incentive constraints that are re-formulated by means of Lemma~\ref{lem:duality}.
%
%that are linearized and relaxed by an additive $\epsilon$ amount.
%
Formally, we define $F_{\epsilon}(\etavec_1, \ldots, \etavec_{n})$ as the maximum of $\ell(\zvec)$ over those $\zvec \in \mcS$ that additionally satisfy the following constraint for every $i \in \N$:
%
\begin{equation}\label{eq:LP2}
	u_i(\zvec)\ge \max\limits_{\phi_i\in\Phi_i}\left(u_i(\phi_i\diamond \zvec)-\etavec_i^\top \cvec_i(\phi_i \diamond \zvec)\right) -\epsilon .
\end{equation}
%
%is the optimal value of the following optimization problem:
%%
%\begin{subequations}\label{eq:LP}
%	\begin{align}
%	\max_{\zvec \in \mcS} & \,\, \ell(\zvec) \quad \textnormal{s.t.}\label{eq:LP1}\\
%	& u_i(\zvec)\ge \max\limits_{\phi_i\in\Phi_i}\left(u_i(\phi_i\diamond \zvec)-\etavec_i^\top \cvec_i(\phi_i \diamond \zvec)\right) -\epsilon\nonumber\\
%	& \hspace{5.45cm} \forall i \in \N. \label{eq:LP2}
%	\end{align}
%\end{subequations}
%
%start from the following optimization problem parameterized by a tuple of Lagrangian multipliers $\etavec_i$, one for each player $i\in[N]$. Define the following function $F_{\ell,\epsilon}(\etavec_1, \ldots, \etavec_{N})$ which computes the maximum of a linear function $\ell:\Delta(\A)\to[0,1]$ over a linearized and $\epsilon$-relaxed constrained over the costs:
%%
%\begin{subequations}\label{eq:LP}
%	\begin{align}
%&	F_{\ell,\epsilon}(\etavec_1,\ldots, \etavec_N):= \max_{\zvec \in \mcS} \ell(\zvec)\,\, s.t.\label{eq:LP1}\\
%	& U_i(\zvec)\ge \max\limits_{\phi_i\in\Phi_i}\left(U_i(\phi_i\diamond \zvec)-\etavec_i^\top \Cvec_i(\phi_i \diamond \zvec)\right) -\epsilon\nonumber\\
%	& \hspace{6cm} \forall i \in N\label{eq:LP2}
%	\end{align}
%\end{subequations}
%
%\[
%F(z,\eta):=\sum\limits_{i} U^i(z)+M\left\{\sum\limits_i\left[ U^i(z)-\max\limits_{\phi^i}\left(U^i(\phi^i z)-\eta^i C(\phi^i z)\right)\right]\right\}.
%\]
%
%Intuitively, when $\zvec$ is an SCE, then the value of the function is the social welfare $\sum_{i \in N} U^i(\zvec)$. On the other hand, when $\zvec$ is \emph{not} an SCE (and M is large enough), then $M\left\{\sum\limits_i\left[ U^i(z)-\max\limits_{\phi^i}\left(U^i(\phi^i z)-\eta^i C(\phi^i z)\right)\right]\right\}$ is negative. Hence, $F(\cdot,\cdot)$ can be positive only when $\zvec$ is \emph{close} to an equilibrium. Moreover, $\lambda$ should be set such that punire the deviations.
%
%\ma{Mostrare formalmente?}\alb{Che cosa?}
%
%
Notice that the $\min$ operator that appears in the right-hand side of Constraints~\eqref{eq:cons_lemmiz} is dropped by adding the outer maximization over the tuples $(\etavec_1,\dots,\etavec_n) \in \D^n$, as the maximum of $\ell$ is always achieved when the right-hand side of such constraints is as small as possible. 


Next, we show that $F_{\epsilon}(\etavec_1, \ldots, \etavec_{n})$ can be computed in polynomial time by means of the \emph{ellipsoid algorithm}.
%
\begin{lemma}\label{lem:efficientF}
	For every tuple $(\etavec_1,\dots,\etavec_n) \in \D^n$, the value of $F_{\epsilon}(\etavec_1,\dots,\etavec_n)$ can be computed in time polynomial in the instance size $|I|$ and $\frac{1}{\epsilon}$.
\end{lemma}

\begin{proof}
	We show that $F_{\epsilon}(\etavec_1,\ldots,\etavec_n)$ can be solved in polynomial time by means of the {ellipsoid algorithm}.
	%
	Let us notice that Constraints~\eqref{eq:LP2} can be equivalently encoded by a set of linear inequalities, one for each player $i\in \N$ and deviation $\phi_i\in vert(\Phi_i)$, where $vert(\Phi_i)$ denotes the set of vertexes of the polytope $\Phi_{i}$ (recall Assumption~\ref{ass:solvablePolytope}).
	%
	Thus, solving $F_{\epsilon}(\etavec_1,\ldots,\etavec_n)$ is equivalent to solving an LP with a (possibly) exponential number of constraints, but polynomially-many variables.
	%
	Such an LP can be solved in polynomial time by means of the ellipsoid algorithm, provided that a polynomial-time separation oracle for the linearized version of Constraints~\eqref{eq:LP2} is available.
	%
	Such an oracle can be implemented by solving the maximization in the right-hand side of Constraints~\eqref{eq:LP2} for a correlated strategy $\zvec\in\Delta_{\A}$ given as input.
	%
	Formally, the separation oracle solves the following problem for each player $i \in \N$:
	\[
		\phi_i^\star\in\arg\max\limits_{\phi_i\in\Phi_i}\left(u_i(\phi_i\diamond\zvec)-\etavec_i^\top\cvec_i(\phi_i\diamond\zvec)\right),
	\]
	which can be done efficiently thanks to Assumption~\ref{ass:solvablePolytope}.
	%
	Then, if the separation oracle finds any $\phi_i^\star$ such that:
	\[
	u_i(\zvec)\ge u_i(\phi^\star_i\diamond\zvec)-\etavec_i^\top\cvec_i(\phi^\star_i\diamond\zvec),
	\]
	it outputs the above inequality as a separating hyperplane to be used in the ellipsoid algorithm.
	%
\end{proof}
%
%
%We can use the previous results of Lemma~\ref{lem:duality} states that a solution to $\max_{(\etavec_1,\ldots,\etavec_N)\in\D^N} F_{\ell,\epsilon} (\etavec_1, \ldots, \etavec_{N})$ would yield an optimal Constrained $\epsilon$-Phi-equilibrium. This is readily seen as the variables $\etavec_i\in\D$ only appear in the constraints of the problem $F_{\ell,\epsilon} (\etavec_1, \ldots, \etavec_{N})$ and the maximum solution is achieved when its constraints are the biggest possible, which happens when the right hand side of Equation~\ref{eq:LP2} is minimized.\ma{rewording}\alb{non si capisce}


Lemma~\ref{lem:efficientF} is \emph{not} enough to complete our algorithm, since we need an efficient way of optimizing $F_\epsilon (\etavec_1,\ldots,\etavec_n)$ over all the tuples of Lagrange multipliers.
%
This problem is non-trivial, since $F_\epsilon (\etavec_1,\ldots,\etavec_n)$ is non-concave in $\etavec_i$.
%
Nevertheless, we show that, by restricting the domain $\D$ of the Lagrange multipliers to a suitably-defined finite ``small'' subset, we can still find a constrained $\epsilon$-Phi-equilibrium whose value of $\ell$ is at least as large as that of any constrained (exact) Phi-equilibrium.
%
This is enough to solve \textsc{ApxCPE}$(1,\epsilon)$.
%s
In particular, we need a finite subset of ``good'' Lagrange multipliers, in the sense of the following definition.
%
%However, this problem is non-concave in $\etavec_i$ and cannot be approximated efficiently (this follows from Theorem~\ref{thm:hardness}).
%Nonetheless, we show that restricting to finite sufficiently small sets of Lagrangian multipliers is sufficient to compute optimal approximate Constrained Phi-equilibrium.
%In particular, we define a finite set of ``good'' Lagrangian multipliers that enjoy the following property.
%
\begin{definition}
	Given any $\delta > 0$, a set $\tilde \D \subseteq \D$ is \emph{$\delta$-optimal} if, for every $\zvec \in \Delta_{\A}$ and $i \in \N$, the following holds:
	%
	\begin{align*}
		\min\limits_{\etavec_i \in \tilde \D}\max\limits_{\phi_i\in\Phi_i}&\left(u_i(\phi_i\diamond \zvec)-\etavec_i^\top \cvec_i(\phi_i \diamond \zvec)\right) \leq \max\limits_{\phi_i \in \Phi^\mcS_i(\zvec)} u_i(\phi_i\diamond\zvec)+\delta.
	\end{align*}
	%	
	%	A set $\bar \D\subseteq \D$ is $\delta$-optimal if for each $\zvec \in \Delta(\A)$ and for each $i\in[N]$ we have
	%	\begin{align}
	%		\min\limits_{\etavec_i \in \bar\D}\max\limits_{\phi_i\in\Phi_i}&\left(U_i(\phi_i\diamond \zvec)-\etavec_i^\top \Cvec_i(\phi_i \diamond \zvec)\right)\\ 
	%		\le &\max\limits_{\phi_i \in \Phi^\mcS_i(\zvec)} U_i(\phi_i\diamond\zvec)+\delta.
	%	\end{align}
\end{definition}
%
Intuitively, thanks to Lemma~\ref{lem:duality}, if we optimize the Lagrange multipliers over a $\delta$-optimal set $\tilde \D \subseteq \D$, instead of optimizing them over $\D$, then we are allowing the players to violate incentive constraints by at most $\delta$.


In the following, we assume that a finite $\delta$-optimal set $\tilde \D \subseteq \D$ is available. 
%
In Section~\ref{sec:Dsets}, se show how to design two particular $\delta$-optimal sets that allow to prove our main results.
%
For ease of presentation, we let 
\[
	L_{\tilde \D, \epsilon}:=\max\limits_{(\etavec_1, \ldots, \etavec_n )\in  \tilde \D^n} F_{\epsilon}(\etavec_1, \ldots, \etavec_n)
\]
be the optimal value of $F_\epsilon (\etavec_1,\ldots,\etavec_n)$ when the Lagrange multipliers are constrained to be in a $\delta$-optimal set $\tilde \D \subseteq \D$.  
%
%Given a set $\bar \D \subseteq \D$, consider the problem:\ma{non definire $L$}\ma{mettere $\epsilon$ a pedice di $F$}
%\[
%L_{\bar\D, \epsilon}:=\max\limits_{(\etavec_1, \ldots, \etavec_N )\in \bar \D^N} F_{\ell,\epsilon}(\etavec_1, \ldots, \etavec_N).
%\]
%
% We observe that $\epsilon$ appears in the problem defining $L_{\D_\delta,\epsilon}$ only in the constraints of $F_{\epsilon}$.
%
% Moreover, a larger value of $\epsilon$ only makes such constraints looser, yielding higher values of $\ell$.
%
Next, we show that, given any $\delta$-optimal set $\tilde \D$ with $\delta \le \epsilon$, the value of $L_{\tilde \D,\epsilon}$ is at least that achieved by constrained (exact) Phi-equilibria, namely $L_{\D,0}$.
%
Formally:
%
%the exact solution (\ie the one with $\epsilon=0$ and the sets of multipliers being $\D$ which is $0$-optimal by Lemma~\ref{lem:duality}).
%
\begin{restatable}{lemma}{deltaOPTProblem}\label{lem:deltaOPT}
	Given any $0 < \delta \leq \epsilon$ and a $\delta$-optimal set $\tilde \D \subseteq \D$, the following holds: $L_{\tilde \D, \epsilon}\ge L_{\D, 0}$.
	%
	% For any $\delta\ge\epsilon$\ma{TBC}, and $\bar\D$ which is $\delta$-optimal we have that $L_{\bar\D, \epsilon}\ge L_{\D, 0}$.
\end{restatable}
%
Intuitively, Lemma~\ref{lem:deltaOPT} is proved by noticing that, provided that $\delta \leq \epsilon$, the incentive constraints violation introduced by using $\tilde \D$ instead of $\D$ is at most $\epsilon$.
%
Moreover, the set of feasible correlated strategies can only expand by allowing incentive constraints to be violated, and, thus, the value of the objective $\ell$ can only increase.  


%\begin{proof}
%	Let $z^*$ be the optimal SCE. It is easy to see that the value of the formulation with $z^*$ is exactly $\sum_{i} U^i(z)$.
%\end{proof}

%\begin{proof}
%	Let $\zvec^\star$ be the Constrained Phi-equilibrium that maximize the social welfare and let $\OPT:=\sum_{i\in[N]} U_i(\zvec^\star)$. 
%	Then, we show that $\max_{\eta\in \bar \D} F_\delta( \eta)$ has value at least OPT.
%	Let $\bar \eta\argmin_{\eta\in \bar \D} \max\limits_{\phi^i}\left(U^i(\phi^i z)-\bar \eta^{i} C(\phi^i z)\right)$.
%	To do so, we show that $z^*$ is feasible for the problem 
%	\begin{subequations}
%		\begin{align}
%		\max_z &\sum\limits_{i} U^i(z) s.t.\\
%		& U^i(z)\ge \max\limits_{\phi^i}\left(U^i(\phi^i z)-\bar \eta^i C(\phi^i z)\right)- \epsilon \forall ....
%		\end{align}
%	\end{subequations}.
%	In particular,
%	\begin{align*} 
%	U^i(z^*) &\ge \max\limits_{\phi^i \in \Phi^i_{\mcS(\zvec^*)}} U^i(z^*) \\
%	&\ge \min_\eta \max_{\phi^i} \left(U^i(\phi^i z^*)- \eta^{i} C(\phi^i z^*)\right)+ \delta\\
%	& = \min_\eta \max_{\phi^i} \left(U^i(\phi^i z^*)- \bar  \eta^{i} C(\phi^i z^*)\right)+ \delta.
%	\end{align*}
%	
%	
%	Hence, $L_{\bar \D,\delta}  \ge F_\delta ( \bar \eta) \ge  \sum_{i \in N} U^i(z^*)= OPT$. 
%	
%	
%	%	Then, we can write $L$ as follows:
%	%	\begin{align}
%	%		L&=OPT+M\left\{OPT-\max\limits_{\phi^i} \left(U^i(\phi^i z^*)-\max\limits_{\eta^i}\eta^i C(\phi^i z^*)\right)\right\}\\
%	%		&=OPT+M\left\{OPT-\max\limits_{\phi^i\, s.t.\, \phi^i z^* \in S} U^i(\phi^i z^*)\right\}\ge OPT,
%	%	\end{align}
%	%where the last inequality holds since $\max\limits_{\phi^i\, s.t.\, \phi^i z^* \in S}U^i(\phi^i z^*)\le U^i(z^*)$
%\end{proof}



%Then, we show that we can bound the value of the Lagrangian multipliers $\eta$.
%let $D=\frac{1}{\rho}$ where $\rho$ is the strictly feasibility parameter.
%
%\begin{lemma}
%	It holds
%%\begin{align}\label{Prog:OPT}
%% L=   \max_{\eta_i \le D} \max_{z\in S} \sum_{i} U^i(z)  +M [ \sum_i [ U^i(z) C(z)-  \max_{\phi^i}  [U^i(z)-\eta_i C(z)]]]  
%%\end{align}
%\begin{align}\label{Prog:OPT}
%L=\max\limits_{\eta\le D}\max\limits_{z\in S} F(z,\eta)
%\end{align}
%\end{lemma}
%
%\begin{proof}
%	First we show that for each $z$, \[ \min_{\eta_i \le D} \max_{\phi^i}  [U^i(z)-\eta_i C(z)] = \max_{\phi^i} [\min_{\eta_i} U^i(z)-\eta_i C(z)]. \]
%	Strong duality like argument. Then, bound Lagrangian multiplier by contradiction.
%	Then, 
%	\begin{align}
%	L&= \max_{z \in S}    \sum_{i} U^i(z)  +M [ \sum_i [ U^i(z)- \min_{\eta_i\le D}  \max_{\phi^i} [U^i(z)-\eta_i C(z)]]] \\
%	&= \max\limits_{\eta\le D}\max\limits_{z\in S} F(z,\eta)
%	\end{align}
%\end{proof}

%\begin{lemma}
%	Suppose $||\tilde\eta-\eta^*||_{\infty}\le \epsilon$, where $\eta^*\in\argmax_\eta\max_{z\in S} F(z,\eta)$ is the optimal parameter. Then,
%	$\argmax_{z\in S} F(z,\tilde\eta) $, is  $\epsilon M N$ optimal and an $N/M$-SCE.
%\end{lemma}
%
%\begin{proof}
%%First, we show that the value of the solution is at least $OPT-\epsilon MN$. 
%Suppose that $(z^*,\eta^*)\in\argmax_{\eta\le D}\max_{z\in S} F(z,\eta)$.
%Since $\|\nabla_\eta F(z,\eta)\|\le MN$ the $F(z,\eta)$ is $MN$ Lipschitz-continuous in $\eta$, then $F(z^*,\tilde\eta)\ge F(z^*,\eta^*)-\epsilon MN\ge OPT-\epsilon MN$.
%Let $\bar z\in\argmax_{z\in S}F(z,\tilde\eta)$ be the solution to the problem in the statement. Since $ \sum_i [ U^i(\bar z) -  \max_{\phi^i}  [U^i(\bar z)-\tilde\eta_i C(\bar z)]] \le 0$ and $F(\bar z,\tilde \eta)\ge F(z^*,\tilde\eta)\ge OPT-\epsilon MN$, it holds that $\sum_i U^i(\bar z)\ge F(\bar z, \tilde \eta)$ and thus that $\sum_{i} U^i(\bar z) \ge OPT-\epsilon MN$ proving the first part of the statement.
%Then, we show that the returned solution $\bar z$ is an $2(N/M+\epsilon N)$-SCE.
%
%Suppose by contradiction that it is not the case. Then the value of $\bar z$ is at most $N-M2(N/M+\epsilon N)\le -\epsilon M N$, contradicting the optimality of $\bar z$.
%
%We have that:
%\begin{align}
%	0\le F(\bar z, \eta)\le &\sum\limits_i U^i(\bar z)+M\left[U^i(\bar z)-\max\limits_{\phi^i}\left(U^i(\phi^i \bar z)-\tilde\eta^i C(\phi^i \bar z)\right)\right]\\
%	\le&\sum\limits_i U^i(\bar z)+M\left[U^i(\bar z)-\max\limits_{\phi^i\, s.t.\, \phi^i z\in S}U^i(\phi^i \bar z)\right],
%\end{align}
%where we used that $U^i(\bar z)-\max\limits_{\phi^i}\left(U^i(\phi^i \bar z)-\tilde\eta^i C(\phi^i \bar z)\right)\ge 0$ for all $i$ and $\max\limits_{\phi^i}\left(U^i(\phi^i \bar z)-\tilde\eta^i C(\phi^i \bar z)\right)\ge \max\limits_{\phi^i\,s.t.\, \phi^i z\in S} U^i(\phi^i z) $. Hence $U^i(\bar z)\ge \max\limits_{\phi^i\, s.t.\, \phi^i z\in S}U^i(\phi^i \bar z)- N/M$.
%
%\end{proof}

Lemma~\ref{lem:deltaOPT} suggests a way of solving \textsc{ApxCPE}$(1,\epsilon)$.
%
% Lemma~\ref{lem:deltaOPT} suggests a way of finding an optimal constrained $\epsilon$-Phi-equilibrium.
%
Indeed, given a finite $\delta$-optimal set $\tilde \D \subseteq \D$ with $\delta \leq \epsilon$, by enumerating over all the tuples of Lagrange multipliers $\etavec_i\in \tilde \D$, one per player $i \in \N$, we can find the desired constrained $\epsilon$-Phi-equilibrium.
%
The following theorem shows that this procedure gives an algorithm for \textsc{ApxCPE}$(1,\epsilon)$ that runs in time polynomial in the instance size, $|\tilde \D|$, and $\frac{1}{\epsilon}$.
%, when the number of players is fixed.
%
%there exists a polynomial algorithm (\ie polynomial in $1/\epsilon$) whenever the number of constraints and number of player is constant.
%
\begin{theorem}\label{th:polyalgo}
	Given a finite $\delta$-optimal set $\tilde \D \subseteq \D$ with $\delta \leq \epsilon$, there exists an algorithm that solves \textsc{ApxCPE}$(1,\epsilon)$ and runs in time polynomial in the instance size $ |I| $, the number $|\tilde \D|$ of elements in $\tilde \D$, and $\frac{1}{\epsilon}$ for every $\epsilon > 0$.
	%	
	%	For any $\epsilon > 0$, given a $\delta$-optimal set $\D_\delta$ with $\delta \leq \epsilon$, there exists an algorithm that solves \textsc{ApxCPE}$(1,\epsilon)$ and runs in time polynomial in the instance size $|I|$ and $\frac{1}{\epsilon}$ when the number of players $n$ is fixed.
	%	
	%	Let $\bar \D$ be a discrete $\delta$-optimal set. Then, there exists a $\poly(|\bar\D|,|I|)$ algorithm that find an $\delta$-SCE with at least the optimal social welfare, where $|I|$ is the size of the instance.\ma{allungare lo statement}
\end{theorem}

\begin{proof}
	The algorithm works by enumerating over all the possible tuples of Lagrange multipliers $\etavec_i\in \tilde \D$, one per player $ i \in \N$.
	%
	These are polynomially many in the size $|\tilde \D|$ when the number of players $n$ is fixed. 
	 %
	For every tuple $(\etavec_1,\ldots,\etavec_n) \in \tilde \D^n$, the algorithm solves $F_{\epsilon}(\etavec_1,\ldots,\etavec_n)$, which can be done in time polynomial in $|I|$ and $\frac{1}{\epsilon}$ thanks to Lemma~\ref{lem:efficientF}.
	 %
	Finally, the algorithm returns the correlated strategy $\zvec \in \Delta_{\A}$ with the highest value of $\ell$ among those computed while solving $F_{\epsilon}(\etavec_1,\ldots,\etavec_n)$.
	%
	It is easy to see that the returned solution solves problem \textsc{ApxCPE}$(1,\epsilon)$ by applying Lemma~\ref{lem:deltaOPT}.
	%
	This concludes the proof.
\end{proof}
%


\subsection{Instantiating the General Algorithm}\label{sec:Dsets}

Next, we show how to build $\delta$-optimal sets $\tilde \D$ that, when they are plugged in the algorithm in Theorem~\ref{th:polyalgo}, allow us to derive our results.
%
In particular, we consider the set:
\[
	\D_\tau := \left\{ \etavec \in\D \, \Big\vert \,  \eta_{j} = k \tau, k \in \left\{0,\dots,\lfloor\nicefrac{1}{\tau \rho} \rfloor \right\}  \, \forall j \in [m] \right\},
\]
%
which is a discretization of $\D$ with a regular lattice of step $\tau \in \mathbb{R}_+$ (notice that $\eta_j$ is the $j$-th component of $\etavec$).
%
%\[
%	\D_\epsilon=\left\{\etavec_i\in\D: \eta_{i,j}=k\epsilon,\,k \in \{0,\dots,\lfloor\nicefrac{1}{\epsilon \rho} \rfloor\},\, \forall j\in[m]\right\},
%\]
%\ie we discretize $\D$ with a regular lattice of size $\epsilon$.
%
By a simple stars and bars combinatorial argument, we have that $|\D_\tau|=\binom{\lfloor\nicefrac{1}{\tau \rho} \rfloor+m}{m}$.
%
Thus, since it holds that $|\D_\tau|=O(\left(\nicefrac{1}{\tau \rho}\right)^{m})$, if the number of constraints $m$ is fixed, $|\D_\tau|$ is bounded by a polynomial in $\nicefrac{1}{\tau \rho}$.
% whenever $m=O(1)$.
%
Moreover, simple combinatorial arguments show that $|\D_\tau| \le (1+m)^{\lfloor\nicefrac{1}{\tau \rho}\rfloor}$.\footnote{See Appendix~\ref{sec:app_optimal} for a formal proof.}
%
% we can use the well known bound $k!\ge (k/3)^k$ to write the following upperbound $\binom{\lfloor\nicefrac{1}{\epsilon \rho} \rfloor+m}{m}\le \left(3\frac{\lfloor\nicefrac{1}{\epsilon \rho} \rfloor+m}{\lfloor\nicefrac{1}{\epsilon \rho}\rfloor}\right)^{\lfloor\nicefrac{1}{\epsilon \rho} \rfloor}\le (1+m)^{\lfloor\nicefrac{1}{\epsilon \rho}\rfloor}$. 
%
Thus, it also holds that $|\D_\tau| = O(m^{\nicefrac{1}{\tau \rho} })$.
%
Notice that the two bounds on $|\D_\tau|$ are non-comparable, and, thus, they give rise to two distinct results, as we show in the following.
%
%
%In the following, we will use the most appropriate one depending on specific assumptions, later ot be discussed.
%
%\ma{Notice that whenever there are a constant number of constraints per player $\D_\epsilon$ has polynomial-size $O(\frac{1}{\epsilon}^{\#constraints N})$. Moreover, the size of the set is upperbounded by $O({\#constraints N}^{\frac{1}{\epsilon}}$.???}



By using the first bound on $|\D_\tau|$, we can show that the set $\D_\tau$ is $\delta$-optimal for $\delta = m \tau$.
%
Formally:
%
\begin{restatable}{lemma}{gridisemopt}\label{lem:bound_1}
	For any $\tau>0$, the set $\D_\tau$ is $\left(\tau m\right)$-optimal.
\end{restatable}
%
Thus, whenever the number $m$ of cost constraints is fixed, Lemma~\ref{lem:bound_1}, together with Theorem~\ref{th:polyalgo}, allows us to provide a polynomial-time algorithm. 
%
% for problem \textsc{ApxCPE}$(1,\epsilon)$ that runs in time polynomial in the instance size and $\frac{1}{\epsilon}$ for every $\epsilon > 0$ when the number $m$ of cost constraints is fixed.
%
Indeed, it is sufficient to apply Theorem~\ref{th:polyalgo} for the $(\tau m)$-optimal set $\D_\tau$ with $\tau := \epsilon / m$ to obtain the following first main result:
%
\begin{corollary}\label{cor:res_1}
	%
	There exists an algorithm that solves problem \textsc{ApxCPE}$(1,\epsilon)$ in time polynomial in $|I|$ and $\frac{1}{\epsilon}$ for every $\epsilon > 0$, when the number $m$ of cost constraints is fixed.
	%	
	%	FPTAS when number of constraint is constant.
	%	In particular, for each $\delta$, setting $\epsilon=\delta/|C|$ and taking $\bar \D=\D_\epsilon$, we obtain a $poly(\D_\epsilon,I)$ algorithm, \emph{i.e.}, $poly( (\delta/ |C|)^{|C|},I)$.
\end{corollary}


On the other hand, by using the second bound on $|\D_\tau|$, we can show that $\D_\tau$ is $\delta$-optimal for $\delta$ depending logarithmically on the number of players' actions.
%
Formally:
%
\begin{restatable}{lemma}{uniform}\label{lem:bound_2}
	For any $\tau>0$, the set $ \D_\tau$ is $\delta$-optimal for $\delta =2\sqrt{{2\tau}\log s / \rho}$, where $s$ is the number of players' actions.
\end{restatable}
%
Lemma~\ref{lem:bound_2} (together with Theorem~\ref{th:polyalgo}) immediately gives us a quasi-polynomial-time for solving \textsc{ApxCPE}$(1,\epsilon)$ for a given constant $\epsilon > 0$.
%
Moreover, its running time becomes polynomial when the number of players' actions is fixed.
%
\begin{corollary}\label{cor:res_2}
	For any constant $\epsilon > 0$, there exists an algorithm that solves \textsc{ApxCPE}$(1,\epsilon)$ in time $O(|I|^{\log s})$.
	%
	Moreover, when the number $s$ of players' actions is fixed, the algorithm runs in time polynomial in $|I|$.
	%
	% In particular, for each $\delta$, setting $k=\log(|A|)/\epsilon^2$ and taking $\bar \D=\hat \D_k$, we obtain a $poly(\hat \D_k,I)$ algorithm, \emph{i.e.}, $poly( |C|^k, I)$. QPTAS. When the number of actions is constant,
	% PTAS.
\end{corollary}
%
Notice that it is in general \emph{not} possible to design an algorithm that runs in time polynomial in $\frac{1}{\epsilon}$, since this would contradict the hardness result in Theorem~\ref{thm:hardness}.
%
% Notice that the quasi-polynomial-time algorithm provided by Corollary~\ref{cor:res_2} does \emph{not} contradict the result in Theorem~\ref{thm:hardness}, since the algorithm works for any constant value of $\epsilon > 0$, while the hardness result holds for an instance dependent $\epsilon_I$ that gets smaller as the number $s$ of players' actions increases.






%Then, we show two different condition under which the set $\D_\epsilon$ (for a suitably defined $\epsilon$) is $\delta$-optimal.
%The first condition is useful to provide a set $\D$ of polynomial-size that is a good approximation of $\D$ whenever the number of constraint is constant, while the second provide a polynomial-size set when the number of \mat{actions} is constant and a quasi-polynomial size in general setting.
% 
%
%\begin{restatable}{lemma}{gridisemopt}\label{lem:bound_1}
%For each $\epsilon>0$, the set $\D_\epsilon$ is $\left(\epsilon m\right)$-optimal.
%\end{restatable}
%
%When the number of constraints is arbitrary large, Theorem~\ref{thm:hardness} shows that it is impossible to find an $\epsilon$-equilibrium in time polynomial in $1/\epsilon$, unless $\mathsf{P}=\mathsf{NP}$.
%Here, we show that this negative result can be partially circumvented.
%In particular, we provide a set of lagrangian multipliers of quasi-polynomial size that will allow us to provide a quasi-polynomial time approximation algorithm. At the same time, our result implies an algorithm that runs in polynomial time for each constant $\epsilon$ when the number of action is constant. 
%
%\begin{restatable}{lemma}{uniform}
%	For each $\epsilon>0$, the set $ \D_\epsilon$ is $\left(2\sqrt{\frac{2\epsilon}{\rho}\log(|\A^i|)}\right)$-optimal.
%\end{restatable}
%
%
%\mat{capire come scrivere i corollari. Per decidere secondo me dobbiamo capire come definire il problema di ottimizazione. Definizione 4.1 mi sembra ragionavole.}
%
%\ma{Definire che FPTAS è in epsilon per l'epsilon che deifniesco il eps-eq}
%
%\begin{corollary}\label{cor:res_1}
%	FPTAS when number of constraint is constant.
%	In particular, for each $\delta$, setting $\epsilon=\delta/|C|$ and taking $\bar \D=\D_\epsilon$, we obtain a $poly(\D_\epsilon,I)$ algorithm, \emph{i.e.}, $poly( (\delta/ |C|)^{|C|},I)$.
%\end{corollary}
%
%
%\begin{corollary}\label{cor:res_2}
%	In particular, for each $\delta$, setting $k=\log(|A|)/\epsilon^2$ and taking $\bar \D=\hat \D_k$, we obtain a $poly(\hat \D_k,I)$ algorithm, \emph{i.e.}, $poly( |C|^k, I)$. QPTAS. When the number of actions is constant,
%	PTAS.
%\end{corollary}














==> src/abstract.tex <==
\begin{abstract}
		The computational study of equilibria involving constraints on players' strategies has been largely neglected.
		%
		However, in real-world applications, players are usually subject to constraints ruling out the feasibility of some of their strategies, such as, \emph{e.g.}, safety requirements and budget caps.
		%
		Computational studies on constrained versions of the Nash equilibrium have lead to some results under very stringent assumptions, while finding constrained versions of the \emph{correlated equilibrium} (CE) is still unexplored.
		%, even though it is much more computationally.
		%
		In this paper, we introduce and computationally characterize \emph{constrained Phi-equilibria}---a more general notion than constrained CEs---in \emph{normal-form games}.
		%
		We show that computing such equilibria is in general computationally intractable,
		%raises considerable computational challenges, 
		and also that the set of the equilibria may \emph{not} be convex, providing a sharp divide with unconstrained CEs.
		%
		Nevertheless, we provide a polynomial-time algorithm for computing a constrained (approximate) Phi-equilibrium maximizing a given linear function,
		%can be done in polynomial time, 
		when either the number of constraints or that of players' actions is fixed.
		%
		Moreover, in the special case in which a player's constraints do \emph{not} depend on other players' strategies, we show that an exact, function-maximizing equilibrium can be computed in polynomial time, while \emph{one} (approximate) equilibrium can be found with an efficient decentralized no-regret learning algorithm.
\end{abstract}

==> src/any.tex <==
\section{Find an SCE}

Prove that 
\[ \min_\lambda \max_{z \in S}  \sum_i [U^i(z)-\lambda_i C z  - \min_{\eta_i} \max_{\phi^i} ( U^i(\phi^i z)-\eta_i C \phi^i z ) ] \ge \max_{z \in S}  \min_\lambda \sum_i [U^i(z)-\lambda_i C z - \min_{\eta_i} \max_{\phi^i} U^i(\phi^i z)-\eta_i C \phi^i z    \]
\[ = \max_{z }   \min_\lambda \sum_i [U^i(z)-\lambda_i C z - \min_{\eta_i} \max_{\phi^i} (U^i(\phi^i z)-\eta_i C \phi^i z)] = \min_\lambda \max_{z } \max_\eta  \sum_i [U^i(z)-\lambda_i C z - \max_{\phi^i} U^i(\phi^i z)-\eta_i C \phi^i z = 0 \]




We have that:
\[ \min_\lambda \max_{z \in S}  \sum_i [U^i(z)-\lambda_i C z - \max_{\phi^i} U^i(\phi^i z)-\lambda_i C \phi^i z  ] = 0\]

Then, 
\[ \max_{z \in S}  \sum_i [U^i(z) - \max_{\phi^i} U^i(\phi^i z)  ] = 0.\]
This implies that there exists an safe solution with

%
%$\sum_t \max_{\phi \in S(z_t)} U^i(\phi(z))\ge \max_{\phi \in S(\sum_t z_t)} \sum_t U^i(\phi(z_t))  $ 
%
%Find a sequence $z_t$, $\lambda_t$ such that
%
%
%
%
%z final is such that 
%$ \max_{\phi feasible} \sum_t \sum_t U^i \phi z -  U^i z  \le \max_{\phi feasible} \sum_t \sum_t U^i \phi z-\lambda_t C \phi z    -  U^i z   \le \sum_t U^i \phi_t z-\lambda_t C \phi_t z    -  U^i z  \le 0$
%
%
%
%$ \max_{\phi} \sum_t  U^i \phi z_t-\lambda_t C \phi z_t    -  U^i z_t  \le \sum_t \max_{\phi} \min_{\lambda} U^i \phi z_t-\lambda C \phi z_t    -  U^i z_t \le 0$.
%
%
%
%

%LP formulation
%
%\begin{align}
% \min &\sum_i [ U^i(z)- \lambda C(z)-  y_{i,a}]  \\
% s.t. & y_{i,a} \le U^i(a',z) - \lambda C(a',z) \forall i,a' ---> \textnormal{utility deviating on a'}. 
%\end{align}





==> src/hardnessOne.tex <==
\section{PPAD-hard find an equilibrium}

\begin{theorem}
	Given an algorithm to find a $SCE$, there exists a polynomial reduction to find a $\epsilon$-NE.
\end{theorem}

\begin{proof}
	Consider a two player game with set of action $A^1$ and $A^2$ and utilities $U^1$ and $U^2$.
	Consider a new game with three players. Player 3 has action $a_{a,a',a''}$ for each $a \in A^1$, $a',a''\in A^2$ and an action $\bar a$. Moreover, $\hat A^1=A^1+\bar a$ and $\hat A^2=A^2 + \bar a$.
	$U^1(\bar a,)=0 $, $U^2(\cdot, \bar a,\cdot)=0 $. 
	$C^3(a,a' ,a_{a,a',a''})=-1$, and  $C^3(a,a'' ,a_{a,a',a''})=1$. All the other costs of player 3 are $0$.
	
	
\end{proof}

==> src/hardnessOptimal.tex <==
%\section{Hardness Result}\label{sec:hard}


%
%
%Given  a linear function $\ell:\Delta(\A)\to[0,1]$, our goal is to approximate the Constrained Phi-equilibria that maximizes a linear combination of the agents' utility. Formally, we define the following problem.
%
%\ma{dire given an instance in prelim}
%\ma{definire i CPE?}
%\begin{definition}
%	Given a set of deviations for each player $\Phi:=\{\Phi_i\}_{i\in[N]}$, a linear function $\ell$, and two values $\alpha, \epsilon\in [0,1]$, \textsc{ApxCPE}$(\alpha,\epsilon)$ is the problem of finding a Costrained $\epsilon$-Phi-equilibrium $\zvec$ such that $\ell(\zvec)\ge \alpha\ell(\zvec^\star)$, where $\zvec^*$ is the optimal Constrained Phi-equilibrium for the linear function $\ell$.
%	%\ma{definire $OPT$... Per ora ho lasciato $L_{\D,0}$.}
%\end{definition}


In order to formally asses the computational challenges of computing constrained Phi-equilibria, we prove the following strong inapproximability result:
%
\begin{restatable}[Hardness]{theorem}{theoremHardness}\label{thm:hardness}
	For any constant $\alpha>0$, the problem \textsc{ApxCPE}$(\alpha,(\alpha/s)^2)$ is \NPHard, where $s$ is the number of players' actions in the instance given as input.
	%	
	%	\textcolor{red}{For any $\alpha>0$, \textsc{ApxCPE}$(\alpha,{\alpha^2}/{|\A|^2})$ is \NPHard\ for any $\alpha>0$ and $0 < \epsilon \leq {\alpha^2}/{|\A|^2}$, where $|\A|$ is the number of ???? of the instance given as input.}
	%
	%even if $\ell$ is the linear function defining the social welfare.
\end{restatable}
%
Intuitively, Theorem~\ref{thm:hardness} states that, for every multiplicative approximation factor $\alpha > 0$, it is \emph{not} possible to find a constrained $\epsilon$-Phi-equilibrium having value of $\ell$ at least a fraction $\alpha$ of its optimal value in time polynomial in $\frac{1}{\epsilon}$.
%
Moreover, as a byproduct of Theorem~\ref{thm:hardness}, we also get the inapproximability up to within any factor of the problem of computing an optimal constrained (exact) Phi-equilibrium. 
%
%\textcolor{red}{As a corollary of Theorem~\ref{thm:hardness}, we also get the inapproximability up to within any factor of the problem of computing an constrained Phi-equilibrium which approximates a linear function $\ell$ of an optimal one.}

%\begin{remark}
%
Notice that the hardness result in Theorem~\ref{thm:hardness} cannot hold for values of $\epsilon$ that are \emph{independent} from the instance size.
%
Indeed, as we prove in Corollary~\ref{cor:res_2} in Section~\ref{sec:optimal}, problem \textsc{ApxCPE}$(1,\epsilon)$ can be solved in quasi-polynomial time in the instance size whenever $\epsilon > 0$ is a given constant.
%
Thus, any \NPHard ness result for \textsc{ApxCPE}$(\alpha,\epsilon)$ would contradict the \emph{exponential-time hypothesis}.\footnote{The exponential-time hypothesis conjectures that solving 3SAT requires at least exponential time.}
%
%\textcolor{red}{Notice that, in order to prove the hardness result in Theorem~\ref{thm:hardness}, it is necessary to use an $\epsilon$ depending on the instance size.
%%
%Indeed, as we prove in the following sections, whenever $\epsilon$ is a constant the problem can be solved in quasi-polynomial time.
%%
%Hence, an hardness result for a constant $\epsilon$ would contradict the exponential-time hypothesis~\citep{boh}.}
% assuming the Exponential-time hypothesis, the problem with constant $\epsilon$ cannot be\NPHard. 
%
%\end{remark}

==> src/nonConvex.tex <==
\section{Challenges of Constrained Phi-equilibria}\label{sec:hard}

In this section, we show that, in cost-constrained normal-form games, Phi-equilibria loose the nice computational properties that they exhibit in unconstrained settings.
%
This is crucially determined by the fact that the set of constrained Phi-equilibria may \emph{not} be convex in general.
%
\begin{proposition}\label{prop:non-convex}
	Given any instance $I := (\Gamma, \Phi)$, the set of constrained Phi-equilibria may {not} be convex.
	%	
	%	The set of constrained Phi-equilibria of a cost-constrained normal-form game may {not} be convex.
\end{proposition}
%
Proposition~\ref{prop:non-convex} is proved by the following example.
%
\begin{example}\label{example}
	%
	Let $\Phi_{\mathsf{ALL}}$ be the set of all the possible deviations
	%as defined above.
	%
	% This set express all possible deviations of player $i$.
	%
	in a two-player game in which each player has two actions, namely $\A_1=\A_2=\{a_0, a_1\}$.
	%
	% $m=1$, i.e. a single cost constraint $\C_1=\C_2$.
	%
	The first player's utility is such that $u_1(a,a')=0$ for all $a \in \A_1$ and $a' \in \A_2$, while the second player's utility is such that $u_2(a_0,a_1)=1$, and $0$ otherwise.
	%
	%
	Both players share the same single cost constraint ($m=1$).
	%
	Their cost functions are defined as $c_i(a_0,a_1)=1$, $c_i(a_0,a_0)=-\frac{1}{2}$, and $c_i(a_1,a)=-1$ for all $a \in \A_2$.
	%
	Notice that the instance defined above satisfies Assumption~\ref{ass:strictly} for $\rho = 1/2$.
	%
	It is easy to see that the correlated strategy $\zvec^1 \in \Delta_{\A}$ such that $\zvec^1[a_0,a_0]=\frac{2}{3}$ and $\zvec^1[a_0,a_1]=\frac{1}{3}$
	%, and $\zvec^1[a_1, a]=0$  otherwise, 
	is a constrained Phi-equilibrium.
	%
	Moreover, the ``pure'' correlated strategy $\zvec^2 \in \Delta_{\A}$ such that  $\zvec^2[a_1,a_0]=1$ is also a constrained Phi-equilibrium.
	%
	However, the combination $\zvec^3=\frac{1}{2} (\zvec^1+\zvec^2)$ is {not} a constrained Phi-equilibrium.
	%
	Indeed, the second player has an incentive to deviate by using a deviation $\phi_2$ such that $\phi_2[a_0,a_1]=1$ and $\phi_2[a_1,a_1]=1$.
	%
	Such a deviation prescribes to play action $a_1$ when $a_0$ is recommended, and to play action $a_1$ when the recommendation is $a_1$.
	%
	% With this deviation the utility of the second player increases. Indeed, 
	Straightforward calculations show that, for every $a \in \A_1$:
	\[
		(\phi_2\diamond \zvec^3)[a, a^\prime] = 
			\begin{cases}
				\frac{1}{2} &\textnormal{if}\quad a^\prime = a_1\\
				0&\textnormal{otherwise},
			\end{cases}
	\]	
	and $u_2(\phi_2\diamond \zvec^3) = \frac{1}{2}>u_2(\zvec^3)= \frac{1}{6}$.
	%
	Moreover, the deviation is safe, since $\phi_2\in\Phi_2^{\mcS}(\zvec^3)$ as $c_2(\phi_2\diamond \zvec^3)=0$.
\end{example}


==> src/openProblem.tex <==
%\section{Discussion on a Related Open Problem}
%
\section{Discussion and Open Problems}


The main positive results that we provide in this paper (Corollaries~\ref{cor:res_1}~and~\ref{cor:res_2}) show that a constrained $\epsilon$-Phi equilibrium maximizing a given linear function can be computed in time polynomial in the instance size and $\frac{1}{\epsilon}$, when either the number of constraints or that of players' actions is fixed.
%
Clearly, this implies that, under the same assumptions, \emph{a} constrained $\epsilon$-Phi-equilibrium can be found efficiently.
%
Moreover, in Section~\ref{sec:easy}, we designed an efficient no-regret learning algorithm that finds \emph{a} constrained $\epsilon$-Phi-equilibrium in settings enjoying special properties (Corollary~\ref{cor:easy_main}).
%
%In our work we found a polynomial algorithm for finding approximate optimal Constrained Phi-equilibria in the case of constant number of actions or constant number of constraints. This clearly implies that we are able to find \emph{any} approximate Constrained Phi-equilibria in polynomial time under such assumptions.
%Furthermore, in Section~\ref{sec:easy} we designed an algorithm that finds an equilibria under the assumption that the costs depends only on the deviations.
%
However, the problem of efficiently computing \emph{a} constrained $\epsilon$-Phi-equilibrium remains open in general. Formally:
%
%
%Formally, we leave the following open problem:
%
\begin{definition}[Open Problem]\label{openProblem}
	Given any instance $I := (\Gamma,\Phi)$, find a constrained $\epsilon$-Phi-equilibrium in time polynomial in the instance size and $\frac{1}{\epsilon}$.
	%	
	%	Given a normal form game, sets $\Phi_i$ of deviations and constraints $\Cvec_i$ for $i\in[N]$ and $\epsilon>0$: find a correlated $\zvec\in\mcS$ in $\poly(1/\epsilon)$ iterations such that $U_i(\zvec)\ge\max_{\phi_i\in\Phi_i(\zvec)}U_i(\phi_i\diamond \zvec)-\epsilon$ for all $i\in[N]$.
\end{definition}
%
Solving the problem above is non-trivial.
%
Proposition~\ref{prop:non-convex} in Section~\ref{sec:hard} proves that the set of constrained $\epsilon$-Phi-equilibria is non-convex, and, thus, solving the problem in Definition~\ref{openProblem} is out of scope for most of the known equilibrium computation techniques.
%
On the other hand, it is unlikely that such a problem is \NPHard.
%
Indeed, a constrained $\epsilon$-Phi-equilibrium always exists and, given any $\zvec \in \Delta_{\A}$, it is possible to verify whether $\zvec$ is an equilibrium or not in polynomial time.
%
Formally, such a problem is said to belong to the $\mathsf{TFNP}$ complexity class, and, thus, standard arguments show that, if the problem is \NPHard, then $\mathsf{NP} = \mathsf{coNP}$~\citep{megiddo1991total}.
%
% See~\cite{bibid} for a similar argument.
%
Thus, one should try to reduce the problem in Definition~\ref{openProblem} to problems in $\mathsf{TFNP}$, such as that of computing a Nash equilibrium.
%
However, while the problem in Definition~\ref{openProblem} shares some properties with that of computing a Nash equilibrium, such as the non-convexity of the set of the equilibria, the former is fundamentally different from the latter, since it exhibits correlation among the players.
%
Thus, a reduction from such a problem to that of computing Nash equilibria would require a gadget to break the correlation among the players, and doing that is highly non-trivial as cost constraints are expressed by linear functions.    




%The following discussion, highlights the non-convexity property of our solution concept and pinpoint the reason for the difficulty of solving Open Problem~\ref{openProblem} in general. Define the function $\Psi(\zvec,\phi_1,\ldots,\phi_N)$ as:
%\[
%	\Psi(\zvec,\phi_1,\ldots,\phi_N):=\sum\limits_{i=1}^N(U_i(\phi_i\diamond \zvec)-U_i(\zvec)),
%\]
%and assume that every set $\Phi_i$ includes the identity transformation so that $\Psi(\zvec,\phi_1,\ldots,\phi_N)\ge0$.
%%
%By defining the function $V(\zvec):=\max_{\phi_i\in\Phi_i^\mcS(\zvec),\forall i\in[N]}\Psi(\zvec,\phi_1,\ldots,\phi_N)$, then the problem of finding a Correlated Phi-equilibria can be restated as finding a correlated strategy $\zvec\in\Delta_{\A}$ such that $V(\zvec)=0$. Equivalently it can be seen as a solution to the following non-convex minimization problem:
%%
%\[
%\min\limits_{\zvec\in\mcS}V(\zvec).
%\]
%%
%The fact that $V(\zvec)$ is non-convex is linked to the fact that the set of zeros of $V$ is non convex (Section~\ref{sec:Nonconvex}).
%%
%and comes from dependence of the inner feasibility set of the inner maximization depends on the outer minimization variable $\zvec$. This is what makes the problem fundamentally more difficult than the case without constraints in which the feasibility set of the inner maximization does not depend on the outer variable $\zvec$. However reducing it to a general non-convex minimization problem seems the wrong approach as we know that there always exists a a correlated strategy of value $0$. The existence of a solution seems to point to consider the class of total search problems $\mathsf{TFNP}$.



==> src/preliminaries.tex <==
\section{Preliminaries}\label{sec:prelim}

In this section, we introduce all the preliminary definitions and results that are needed in the rest of the paper.


\subsection{Cost-constrained Normal-form Games}

%We let $\N := \{1,\ldots, n\}$ be the set of players 
%
In a \emph{normal-form game}, there is a finite set $\N := \{1,\ldots, n\}$ of $n$ players.
%
Each player $i \in \N$ has a finite set $\A_i$ of actions available, with $s := |\A_i|$ for $i \in \N$ being the number of players' actions.\footnote{For ease of presentation, in this paper we assume that all the players have the same number of actions. All the results can be easily generalized to the case of different numbers of actions.}
%
We denote by $\avec \in \A := \bigtimes_{i \in \N} \A_i$ an action profile specifying an action $a_i$ for each player $i \in \N$.
%
Moreover, for $i \in \N$, we let $\avec_{-i} \in \A_{-i} := \bigtimes_{j \neq i \in \N} \A_i$ be an action profile of all players other than $i$, while $(a,\avec_{-i})$ is the action profile obtained by adding $a \in \A_i$ to $\avec_{-i}$.
%
%
%Moreover, we denote the set of actions of all players except player $i$ by $A^{-i}:=\times_{j\in[N], j\neq i}\A^j$ and the set of all possible action profiles as $\A:=\times_{j\in[N]}\A^j$.
%%
%As common in normal form games we denote as $\Delta(B)$ the set of distributions over any finite set $B$
%
Finally, we let $u_i:\A\to[0,1]$ be the utility function of player $i\in \N$, with $u_i(\avec)$ being the utility perceived by that player when the action profile $\avec\in\A$ is played.




%We denote by $\zvec \in \Delta_{\A}$ a \emph{correlated strategy} defined over the set of all the actions profiles, with $\zvec[\avec]$ denoting the probability assigned to $\avec \in \A$.\footnote{In this paper, given a finite set $X$, we denote by $\Delta_X$ the set of all the probability distributions defined over the elements of $X$.}
%%
%% We let $u_i:\A\to[0,1]$ be the utility perceived by player $i\in N$ when an action profile $\avec\in\A$ is played.
%%
%Then, with an abuse of notation, for every player $i\in \N$, we use $u_i(\zvec)$ to denote player $i$'s expected utility when the action profile played by the players is drawn according to a distribution $\zvec \in \Delta_{\A}$.
%%
%In particular, it holds $u_i(\zvec):=\sum_{\avec\in\A}u_i(\avec)  \zvec[\avec]$.
%
% $U_i:\Delta(\A)\to[0,1]$ be the expected utility perceived by the $i$-th player when actions for all players are drown from the a correlated distribution in $\Delta(\A)$. Formally, this is defined as $U_i(\zvec):=\sum_{\avec\in\A}u_i(\avec)\zvec[\avec]$.


We extend classical normal-form games by considering the case in which each player $i \in \N$ has $m_i$ \emph{cost functions}, namely $c_{i,j}: \A \to [-1,1]$ for $j \in [m_i]$.\footnote{In this paper, given some $x \in \mathbb{N}_{>0}$, we let $[x] := \{ 1,\ldots,x \}$ be the set of the first $x$ natural numbers.}
%
Each player $i \in \N$ is subject to $m_i$ \emph{constraints}, which require that all player $i$'s costs are less than or equal to zero.\footnote{Since $\zvec\in\Delta_{\A}$, we can assume w.l.o.g. that all the constraints are of the form $\leq 0$, as any constraint can always be cast in such a form by suitably manipulating the cost function $c_{i,j}$.}
%bounding their expected costs.
%
% W.l.o.g., we assume that such constraints require that .\footnote{Given that $\zvec\in\Delta_{\A}$, a constraint can always be expressed as $\preceq \zerovec$ by adding suitable constants to each cost function $c_{i,j}$.}
%
For ease of notation, we assume w.l.o.g. that all players have the same number of constraints, namely $m := m_i$ for all $i \in \N$.
%
Moreover, we encode the costs of player $i \in \N$ by a vector-valued function $\cvec_i:\A\to[-1,1]^{m}$ such that, for every $\avec \in \A$, the $j$-th component of the vector $\cvec_i(\avec)$ is $c_{i,j}(\avec)$.
%
% As for utilities, we abuse notation and write $\cvec_i(\zvec):=\sum_{\avec\in\A}\cvec_i(\avec)\zvec[\avec]$ to denote the vector of player $i$'s expected costs under a correlated strategy $\zvec \in \Delta_{\A}$.
%
%
%Furthermore, each player $i$ has $m_i$ constraints $c_{i,j}:\A\to[-1,1]$ for $j\in[m_i]$, which map each tuple of actions to a vector of $m_i$ costs. For ease of notation we can assume that $m_i=m$ for all $i\in[N]$, by possibly adding fictitious costs to each player.
%Moreover we can represent the costs for each player $i$ as vector $\cvec_i:\A\to[-1,1]^{m}$, where, for every action $\avec$ in $\A$, the $j$-th component of $\cvec_i(\avec)$ is $c_{i,j}(\avec)$. Similarly to utilities we can define the vector of expected costs $\Cvec_i:\Delta(\A)\to[-1,1]^m$ where for each correlated strategy $\zvec\in\Delta(\A)$ as $\Cvec_i(\zvec):=\sum_{\avec\in\A}\cvec_i(\avec)\zvec[\avec].$


%Each player $i \in \N$ is subject to $m$ \emph{constraints} bounding their expected costs.
%%
%W.l.o.g., we assume that such constraints are of the form $\cvec_i(\zvec) \preceq \zerovec$.\footnote{Given that $\zvec\in\Delta_{\A}$, a constraint can always be expressed as $\preceq \zerovec$ by adding suitable constants to each cost function $c_{i,j}$.}
%
% W.l.o.g., we assume that such constraints are of the form $\cvec_i(\zvec) \preceq \zerovec$.\footnote{Given that $\zvec\in\Delta_{\A}$, a constraint can always be expressed as $\preceq \zerovec$ by adding suitable constants to each cost function $c_{i,j}$.}
%
%We define $\mcS \subseteq \Delta_{\A}$ as the set of \emph{safe} correlated strategies, which are those satisfying the cost constraints for all players.
%%
%Formally:
%\[
%	\mcS:=\left\{ \zvec\in\Delta_{\A} \mid \cvec_i(\zvec)\preceq \zerovec \quad \forall i\in \N \right\}.
%\]
%%
%In the following, we assume w.l.o.g. that $\mcS \neq \varnothing$.
%
%
%Without loss of generality we can define the set of safe correlated strategies $\mcS$ as the correlated strategies that have non-positive cost, which means for each correlated strategy $\zvec\in \mcS$, the resulting vector of costs is non-positive in all components.
%Namely:
%\[
%\mcS:=\{\zvec\in\Delta(\A)\,|\,\Cvec_i(\zvec)\preceq \zerovec, \forall i\in[N]\},
%\]
%where $\preceq$ denotes the element wise ordering between vectors.
%We can naturally assume that $\mcS$ is non-empty.


\paragraph{Correlated Strategies}
%
In this paper, we deal with solution concepts defined by correlated strategies.
%
A \emph{correlated strategy} $\zvec \in \Delta_{\A}$ is a probability distribution defined over the set of actions profiles, with $\zvec[\avec]$ denoting the probability assigned to $\avec \in \A$.\footnote{In this paper, given a finite set $X$, we denote by $\Delta_X$ the set of all the probability distributions defined over the elements of $X$.}
%
% We let $u_i:\A\to[0,1]$ be the utility perceived by player $i\in N$ when an action profile $\avec\in\A$ is played.
%
With an abuse of notation, for every player $i\in \N$, we let $u_i(\zvec)$ be player $i$'s expected utility when the action profile played by the players is drawn from $\zvec \in \Delta_{\A}$.
%
In particular, it holds $u_i(\zvec):=\sum_{\avec\in\A}u_i(\avec)  \zvec[\avec]$.
%
Similarly, we let $\cvec_i(\zvec):=\sum_{\avec\in\A}\cvec_i(\avec)\zvec[\avec]$ be the vector of player $i$'s expected costs,
% under a correlated strategy $\zvec \in \Delta_{\A}$.
%
so that player $i$'s constraints can be compactly written as $\cvec_i(\zvec) \preceq \zerovec$.
%
Finally, we define $\mcS \subseteq \Delta_{\A}$ as the set of \emph{safe} correlated strategies, which are those satisfying the cost constraints of all players.
%
Formally:
\[
	\mcS:=\left\{ \zvec\in\Delta_{\A} \mid \cvec_i(\zvec)\preceq \zerovec \quad \forall i\in \N \right\}.
\]
%
In the following, we assume w.l.o.g. that $\mcS \neq \varnothing$.


\subsection{Constrained Phi-equilibria}




We generalize the notion of Phi-equilibria~\citep{greenwald2003general} to cost-constrained normal-form games.
%
Such equilibria are defined as correlated strategies $\zvec \in \Delta_{\A}$ that are robust against a given set $\Phi$ of players' deviations, in the sense that, if a mediator draws an action profile $\avec \in \A$ according to $\zvec$ and recommends to play action $a_i$ to each player $i \in \N$, then no player has an incentive to deviate from their recommendation by selecting a deviation in $\Phi$.   


For every $i \in \N$, we let $\Phi_i$ be the set of player $i$'s \emph{deviations}, \emph{i.e.}, linear transformations $\phi_i : \A_i \to \Delta_{\A_i}$ that prescribe a probability distribution over player $i$'s actions for every possible action recommendation.
%
For ease of notation, we encode a deviation $\phi_i$ by means of its matrix representation.
%
Formally, an entry $\phi_i[b,a]$ of the matrix represents the probability assigned to action $a \in \A_i$ by $\phi_i(b)$.
%
We denote the set of all the possible deviations by $\Phi := \{\Phi_i\}_{i\in \N}$.




Given a correlated strategy $\zvec \in \Delta_{\A}$ and a deviation $\phi_i \in \Phi_i$, we define $\phi_i\diamond \zvec$ as the \emph{modification} of $\zvec$ induced by $\phi_i$, which is a linear transformation that can be expressed as follows in terms of matrix representation:
\[
	(\phi_i\diamond \zvec)[a_i,\avec_{-i}] := \sum\limits_{b\in\A_i}\phi_i[b,a_{i}]\zvec[b,\avec_{-i}],
\]
for every $a_i \in \A_i$ and $\avec_{-i} \in \A_{-i}$.
%
Moreover, given a set $\Phi_i$ of deviations of player $i \in \N$, in the following we denote by $\Phi_{i}^{\mcS}(\zvec) := \left\{ \phi_i\in\Phi_i \mid \phi_i\diamond \zvec\in \mcS \right\}$ the set of \emph{safe deviations} for player $i$ at a given correlated strategy $\zvec\in\Delta_{\A}$.
%
%Let $\Phi$ be the set of possible deviations, i.e. $\Phi=\{\Phi_i\}_{i\in[N]}$, where each $\Phi_i$ is a subset of linear transformations $\phi_i:\A^i\to\Delta(\A^i)$ that prescribe a deviation from an action $a\in\A^i$ to a distribution over the actions $\A^i$. For ease of notation we represent a deviation $\phi_i$ with its matrix representation. More formally, we write $\phi_i[b,a]$ be the probability of playing action $a$ when action $b$ is recommanded. With this notation the modification $\phi_i\diamond \zvec$ is a linear function and can be expressed as:
%\[
%(\phi_i\diamond \zvec)[a_i,\avec_{-i}] := \sum\limits_{b\in\A^i}\phi_i[b,a_{i}]\zvec[b,\avec_{-i}].
%\]



We are now ready to provide our definition of \emph{constrained Phi-equilibria} in cost-constrained normal-form games.
%
\begin{definition}[Constrained $\epsilon$-Phi-equilibria]
	% Given a set $\Phi := \{\Phi_i\}_{i\in \N}$ of deviations, let $\Phi_{i}^{\mcS}(\zvec) := \left\{ \phi_i\in\Phi_i \mid \phi_i\diamond \zvec\in \mcS \right\}$ be the of constrained deviations at any correlated strategy $\zvec\in\Delta_{\A}$.
	%
	Given a set $\Phi := \{ \Phi_i \}_{i \in \N}$ of deviations and an $\epsilon>0$, a \emph{constrained $\epsilon$-Phi-equilibrium} is a safe correlated strategy $\zvec\in\mcS$ such that, for all $i\in \N$, the following holds:
	%
	\[
	 u_i(\zvec)\ge u_i(\phi_i\diamond \zvec)-\epsilon\quad\forall\phi_i\in \Phi^\mcS_i(\zvec).
	\]
	%
	A \emph{constrained Phi-equilibrium} is defined for $\epsilon = 0$.
	%	
	%	Let $\Phi_{i}^{\mcS}(\zvec):=\{\phi_i\in\Phi_i\,|\,\phi_i\diamond \zvec\in \mcS\}$ be the set of constrained deviations at a specific correlated strategy $\zvec\in\Delta(\A)$.
	%	%
	%	For any $\epsilon>0$, a Constrained $\epsilon$-Phi-equilibrium is defined as a correlated strategy $\zvec\in\mcS$ such that for all $i\in[N]$:
	%	%
	%	\[
	%	U_i(\zvec)\ge U_i(\phi_i\diamond \zvec)-\epsilon\quad\forall\phi_i\in \Phi^\mcS_i(\zvec).
	%	\]
\end{definition}



\subsection{Computing Constrained Phi-equilibria}


In the following, we formally introduce the computational problem that we study in the rest of the paper.

We denote by $I := (\Gamma,\Phi)$ an instance of the problem, where the tuple $\Gamma := (\N,\A,\{u_i\}_{i\in \N}, \{c_{i,j} \}_{i\in \N,j\in [m]})$ is a cost-constrained normal-form game and $\Phi := \{ \Phi_i \}_{i \in \N}$ is a set of deviations.
%
Moreover, we let $|I|$ be the size (in terms of number of bits) of the instance $I$.
%
We assume that the number $n$ of players is fixed, so that $|I|$ does \emph{not} grow exponentially in $n$.\footnote{Notice that the size of the representation of a normal-form game is $O(s^n)$, and, thus, exponential in $n$. Any algorithm that runs in time polynomial in such instance size is \emph{not} computationally appealing, as even its input has size exponential in $n$. For this reason, we focus on the case in which $n$ is fixed, and, thus, the instance size does \emph{not} grow exponentially with $n$.}
%
We also make the following assumption on how the sets of deviations are represented:
% specified in the representation of an instance $I$.
%
% We first introduce a very natural assumption on the set of possible deviations $\Phi_i$.
%
\begin{assumption}\label{ass:solvablePolytope}
	For every $i \in \N$, the set $\Phi_i$ is a polytope encoded by a finite of linear inequalities.\footnote{Notice that, since each $\phi_i \in \Phi_i$ is represented as a matrix, a linear inequality is expressed as $\sum_{b,a \in \A_i} M[b,a] \phi_i[b,a]\le d$, for some matrix $M$ and scalar $d$.}
	%	
	%	$\Phi_i$ is a polytope for all $i\in[N]$ encoded by a finite set of linear inequalities of the form $\sum_{a,b} M[a,b] \phi[a,b]\le d$ for two given M and d.
\end{assumption}
%
Let us remark that, in games without constraints, this assumption is met by all the sets $\Phi$ which determine the classical notions of Phi-equilibria~\citep{greenwald2003general}.
%
%We remark that in the setting without constrains, this assumption is met by all the  sets $\Phi$ which give arise to all the main solution concepts~\cite{greenwald2003general}.


Next, we formally define our computational problem:
%
\begin{definition}[\textsc{ApxCPE}$(\alpha,\epsilon)$]\label{def:probelm}
	%
	For any $\alpha,\epsilon > 0$, we define \textsc{ApxCPE}$(\alpha,\epsilon)$ as the problem of finding, given an instance $I := (\Gamma,\Phi)$ and a linear function $\ell : \Delta_{\A} \to \mathbb{R}$ as input, a constrained $\epsilon$-Phi-equilibrium $\zvec \in \Delta_{\A}$ such that $\ell(\zvec)\ge \alpha\ell(\zvec')$ for all constrained Phi-equilibria $\zvec' \in \Delta_{\A}$.
	%	
	%	Given a set of deviations for each player $\Phi:=\{\Phi_i\}_{i\in[N]}$, a linear function $\ell$, and two values $\alpha, \epsilon\in [0,1]$, \textsc{ApxCPE}$(\alpha,\epsilon)$ is the problem of finding a Costrained $\epsilon$-Phi-equilibrium $\zvec$ such that $\ell(\zvec)\ge \alpha\ell(\zvec^\star)$, where $\zvec^*$ is the optimal Constrained Phi-equilibrium for the linear function $\ell$.
	%	%\ma{definire $OPT$... Per ora ho lasciato $L_{\D,0}$.}
\end{definition}
%
Intuitively, \textsc{ApxCPE}$(\alpha,\epsilon)$ asks to compute a constrained $\epsilon$-Phi-equilibrium whose value for the linear function $\ell$ is at least a fraction $\alpha$ of the maximum value which can be achieved by an (exact) constrained Phi-equilibrium.


In order to ensure that an instance of our problem is well defined, we make the following ``Slater-like'' assumption on how the players' cost constraints are defined.
%
\begin{assumption} \label{ass:strictly}
	For every correlated strategy $\zvec\in\Delta_{\A}$, player $i\in \N$, and index $j\in[m]$, there exists $\phi^\circ_i\in\Phi_i^\mcS(\zvec)$:
	\[ 
		c_{i,j}(\phi^\circ_i \diamond \zvec)\le -\rho,
	\]
	where $\rho>0$ and $1/\rho$ is $O(\textnormal{poly}(|I|))$, with $\textnormal{poly}(|I|)$ being a polynomial function of the instance size $|I|$.
\end{assumption}
%
In Assumption~\ref{ass:strictly}, the condition $\rho > 0$ is required to guarantee the existence of a constrained Phi-equilibrium (see Theorem~\ref{thm:existence}) and that the sets $\Phi_i^\mcS(\zvec)$ are non-empty (otherwise our solution concept would be ill defined).
%
Moreover, the second condition on $\rho$ in Assumption~\ref{ass:strictly} is equivalent to requiring that our algorithms run in time polynomial in $\frac{1}{\rho}$.
%
%\textcolor{red}{Bisogna mettere dei cetrioli sulla seconda assunzione.}
% \textcolor{red}{Moreover, the second condition on $\rho$ is the weaker assumption needed to avoid some technicalities in the derivation of our results.}
%
%Assumption~\ref{ass:strictly} is required to prove the existence of Constrained Phi-equilibrium and that the set $\Phi_i^\mcS(\zvec)$ is non-empty. Moreover, the polynomial relation between $1/\rho$ and the instance size $|\I|$ is the looser assumption required to avoid computational technicalities and to avoid that $\rho\to0$ for which the solution concept might be ill defined. 


Assumption~\ref{ass:strictly} also allows us to prove the existence of our equilibria, by showing that the constrained Nash equilibria introduced by~\citet{altman2000constrained}, which always exist under Assumption~\ref{ass:strictly}, are also constrained Phi-equilibria.
%
% With these assumptions we can readily prove the existence of our solution concept.
%
\begin{restatable}{theorem}{existence}\label{thm:existence}
	Given a cost-constrained normal-form game $\Gamma$ and a set $\Phi$ of deviations, if Assumption~\ref{ass:strictly} is satisfied, then $\Gamma$ admits a constrained Phi-equilibrium. 
	%
	% There exists a Constrained Phi-equilibrium for any deviation set $\Phi$ and costs $\{\Cvec_i\}_{i\in[N]}$ such that Assumption~\ref{ass:strictly} holds.
\end{restatable}


\subsection{Relation with Unconstrained Phi-equilibria}\label{sec:prelim_relations}

We conclude the section by discussing the relation between our constrained Phi-equilibria and classical equilibrium concepts for unconstrained games.
%
% In particular, our equilibria include the constrained versions of classical equilibrium notions based on correlation.
%
%In this section we discuss the relation and differences of our definition to the standard definition of Phi-equilibria.
%
% First we introduce the two most common sets of deviations that include many common definition of equilibria in Normal Form Games in absence of costs constraints.



\paragraph{Correlated Equilibrium}
%
When there are no constraints, the \emph{correlated equilibrium} (CE)~\citep{aumann1974subjectivity} is a special case of Phi-equilibrium.
%
As shown by~\citet{greenwald2003general}, the CE is obtained when the sets $\Phi_i$ contain all the possible deviations. 
%
Formally, the CE is defined by the set $\Phi_{\textsc{all}} := \{ \Phi_{i,\textsc{all}} \}$ of deviations such that:
\[
	\Phi_{i,\textsc{all}} := \left\{\phi_i  \, \Big\vert \, \sum_{a\in\A_i}\phi_i[b,a]=1 \quad \forall b\in\A_i\right\}.
\]
%
%
%
%\[
%\Phi_{i,\textnormal{ALL}} := \left\{\phi_i[b,a]\in[0,1]: \sum_{a\in\A^i}\phi_i[b,a]=1,\, \forall b\in\A^i\right\}.
%\]
%This set encodes all the possible deviations strategies. In absence of costs constraints, the set of Phi-equilibria when using this set of deviations are equivalent to the set of \emph{Correlated Equilibria}~\cite{greenwald2003general}.\ma{}



\paragraph{Coarse Correlated Equilibrium}
%
The \emph{coarse correlated equilibrium} (CCE)~\citep{moulin1978strategically} is a special (unconstrained) Phi-equilibrium whose set of deviations is $\Phi_{\textsc{CCE}} := \{ \Phi_{i,\textsc{CCE}} \}_{i \in \N}$ such that:
\[
	\Phi_{i,\textsc{CCE}} := \left\{ \phi_i \,\Big\vert \,\exists \boldsymbol{h} \in \Delta_{\A_i} : \phi_i[b,a] = \boldsymbol{h}[a] \,\,\, \forall b,a \in \A_i \right\}.
\]
%
Intuitively, such sets contain all the possible deviations that prescribe the same probability distribution independently of the received action recommendation.
% do \emph{not} depend on the received recommendation.
%
%%
%Consider now the set of deviations defined as:
%\[
%\Phi_{i,\textnormal{CCE}}:=\left\{\phi_i[b,a]=c_a\in[0,1]\,\forall b\in\A: \sum_{a\in\A^i}c_a=1\right\}.
%\]
%This set encodes all possible deviations that do not depend on the recommendation received by the player. When we consider such set for the deviations in absence of costs constraints we recover the definition of \emph{Coarse Correlated Equilibrium}~\cite{greenwald2003general}.

Thus, our constrained Phi-equilibria include the generalization of CEs and CCEs to cost-constrained games.

Our definition of constrained Phi-equilibrium needs to employ ``mixed'' deviations that map action recommendations to probability distributions over actions.
%
This is necessary in presence of constraints.
%
Instead, without them, one can simply consider ``pure'' deviations that map recommendations to actions deterministically~\cite{greenwald2003general}.
%
%In our definition of Constrained Phi-equilibrium needs to use the set of ``mixed'' deviations. In literature, the sets are usually comprised of a discrete of ``pure'' deviations. In the absence of constraints considering ``mixed'' or ``pure'' is equivalent, however in the presence of constraints makes it necessary to consider mixed deviations. 

%However we need to consider the convex polytope generated by such deviations since it might be the case that, in the presence of constraints, the hyperplanes of such constraints cut the 


%
%
%\ma{Definire set dei C-CE, C-CCE, ecc}
%\ma{Spiegare perhcè non si possono prendere i $\Phi_{INT}$ della Amy}
%\ma{Spostare qui la definizione del problema 4.1?}




==> src/specialCase.tex <==
\section{A Special Case: Deviation-dependent Costs}\label{sec:easy}

We complete our computational study of constrained Phi-equilibria by considering a special case in which player $i$'s costs associated to a deviation $\phi_i$ only depend on $\phi_i$ and \emph{not} on the (overall) modified correlated strategy $\phi_i\diamond\zvec$.




We consider instances satisfying the following assumption.
%
\begin{assumption}\label{ass:cce}
	For every player $i\in \N$ and player $i$'s deviation $\phi_i\in\Phi_i$, there exists a function $\tilde\cvec_i: \Phi_i\to[-1,1]^m$ such that $\tilde\cvec_i(\phi_i) :=\cvec_i(\phi_i \diamond\zvec)$ for every $\zvec \in \Delta_{\A}$.
	%
	% it holds that there exists $\tilde\Cvec_i:\Phi_i\to[-1,1]^m$ such that $\tilde\Cvec_i(\phi_i)=\Cvec_i(\phi_i \diamond\zvec)$.
\end{assumption}
%
%Thus, with abuse of notation, we can write $\Cvec_i(\phi_i\diamond\zvec)\equiv\tilde\Cvec_i(\phi_i)$ whenever Assumption~\ref{ass:cce} holds.
%
Notice that, whenever Assumption~\ref{ass:cce} holds, the set $\Phi_i^\mcS(\zvec)$ of safe deviations does \emph{not} depend on $\zvec$.
%
Thus, in the rest of this section, we write w.l.o.g. $\Phi_i^\mcS$ rather than $\Phi_i^\mcS(\zvec)$.
%
% We remark that Assumption~\ref{ass:cce} is in general a joint property of the set $\Phi_i$ and the costs $\Cvec_i$.



A positive effect of Assumption~\ref{ass:cce} is that it recovers the convexity of the set of constrained Phi-equilibria, rendering them more akin to unconstrained ones.
%
Formally:
%
\begin{restatable}{proposition}{convex}\label{thm:convex}
	For instances $I := (\Gamma,\Phi)$ satisfying Assumption~\ref{ass:cce}, the set of constrained $\epsilon$-Phi-equilibria is convex.
	% whenever Assumption~\ref{ass:cce} holds.
	%
	% The set of constrained $\epsilon$-Phi-equilibria is convex whenever Assumption~\ref{ass:cce} holds.
\end{restatable}
%
%
Proposition~\ref{thm:convex} suggests that constrained Phi-equilibria are much more computationally appealing under Assumption~\ref{ass:cce} than in general, as we indeed show in the rest of this section.




% After formally introducing the model studied in this section, in 
%
First, in Section~\ref{sec:easy_optimal}, we show that \textsc{ApxCPE}$(1,0)$ admits a polynomial-time algorithm under Assumption~\ref{ass:cce}.
%
Then, in Section~\ref{sec:easy_learning}, we design a no-regret learning algorithm that efficiently computes \emph{one} constrained $\epsilon$-Phi equilibrium with $\epsilon= O(\nicefrac{1}{\sqrt{T}})$ as the number of rounds $T$ grows.
%
Finally, in Section~\ref{sec:easy_cce}, we provide a natural example of constrained Phi-equilibria satisfying Assumption~\ref{ass:cce}.
%
%
%
%We complete the study of Constrained Phi-equilbria by considering a special case, in wich the costs only depend on the deviation $\phi_i$ chosen by the $i$-th player and not by the ovarall modified correlated strategy $\phi_i\diamond\zvec$. At the end of the section\ma{o meglio subito?} we will give a natural example that satisfies such hypothesis.





\subsection{A Poly-time Algorithm for Optimal Equilibria}\label{sec:easy_optimal}



We prove that, whenever Assumption~\ref{ass:cce} holds, the problem of computing an (exact) Phi-equilibrium maximizing a given linear function can be solved in polynomial time.
%
This is done by formulating the problem as an LP with polynomially-many variables and exponentially-many constraints, which can be solved by means of the ellipsoid method, similarly to how we compute $F_\epsilon(\etavec_1,\ldots\etavec_n)$ in Section~\ref{sec:optimal} (see the proof of Lemma~\ref{lem:efficientF}). 
%
% The problem of finding an optimal Constrained Phi-equilibrium can readily written as an LP which we can solve with the ellipsoid algorithm, similarly to Lemma~\ref{lem:efficientF} we can state the following:
%
Formally:
%
\begin{restatable}{theorem}{optimalsimple}\label{th:optimal_MCCCE}
	Restricted to instances $I := (\Gamma,\Phi)$ which satisfy Assumption~\ref{ass:cce}, \textsc{ApxCPE}$(1,0)$ admits a polynomial-time algorithm.
	%
	%then we can find an exact constrained Phi-equilibrium in polynomial time.
\end{restatable}



\subsection{An Efficient No-regret Learning Algorithm}\label{sec:easy_learning}


Next, we show how Assumption~\ref{ass:cce} allows us to find a constrained $\epsilon$-Phi-equilibrium by means of a polynomial-time decentralized no-regret learning algorithm.
%
Our algorithm is based on the Phi-regret minimization framework introduced by~\citet{greenwald2003general}, which needs to be extended in order to be able to work with polytopal sets $\Phi_i^\mcS$ of safe deviations, rather than finite sets of ``pure'' deviations.
%
% In this section we will show how to find approximate Constrained Phi-equilibria in a simple decentralized manner when Assumption~\ref{ass:cce} holds.
% The techniques used here are related to the no Phi-regret learning literature.

\begin{algorithm}[!htp]\caption{{Learning a Constrained $\epsilon$-Phi-equilibria}}\label{alg:noregret}
	\begin{algorithmic}[1]
		\REQUIRE Regret minimizers $\mfR_i$ for the sets $\Phi_i^\mcS$, for $i\in \N$
		\STATE Initialize the regret minimizers $\mfR_i$
		\FOR{$t=1, \ldots, T$}
		\FOR{each player $i \in \N$}
		\STATE $\phi_{i,t}\gets \mfR_i.\textsc{Recommend}()$\label{lin:recc}
		\STATE Play according to a distribution $\xvec_{i,t}\in\Delta_{\A_i}$ s.t. $$\xvec_{i,t}[a] = \sum_{b\in\A_i}\phi_{i,t}[b,a]\xvec_{i,t}[b] \quad \forall a\in\A_i$$
		\ENDFOR
		\STATE $\zvec_t\gets\otimes_{i\in \N} \, \xvec_{i,t}$
		\STATE $\mfR_i.\textsc{Observe}( \phi_i \mapsto u_i(\phi_i \diamond \zvec_t) )$\label{lin:obs}
		\ENDFOR
		\STATE \textbf{return} $\bar\zvec_T := \frac{1}{T}\sum_{t=1}^T\zvec_t$
	\end{algorithmic}
\end{algorithm}


Algorithm~\ref{alg:noregret} outlines our no-regret algorithm.
%
It instantiates a regret minimizer $\mfR_i$ for the polytope $\Phi_i^\mcS$ for each $i\in \N$.
%
$\mfR_i$ is an object that, at each round $t \in [T]$, recommends a safe deviation $\phi_{i,t} \in \Phi_i^\mcS$ to player $i$ (Line~4 of Algorithm~\ref{alg:noregret}), and, then, observes a function $\phi_i \mapsto u_i(\phi_i \diamond \zvec_t)$ that specifies the utility that would have been obtained by selecting any safe deviation $\phi_i \in \Phi_i^\mcS$ at round $t$  (Line~8 of Algorithm~\ref{alg:noregret}).
%
$\mfR_i$ guarantees that the regret $R_i^T$ cumulated by player $i$ over $[T]$ grows sublinearly, \ie $R_i^T = o(T)$, where:
\[
	R_i^T := \max_{\phi_i \in \Phi_i} \sum_{t=1}^T  u_i(\phi_i\diamond\zvec_t)-\sum_{t=1}^T u_i(\phi_{i,t}\diamond\zvec_t),
\]
which is how much player $i$ loses by selecting $\phi_{i,t}$ at each $t$ rather than choosing the same best-in-hindsight deviation at all rounds.
%
Notice that, by taking inspiration from the Phi-regret framework~\citep{greenwald2003general}, given a recommended deviation $\phi_{i,t}$, player $i$ actually plays according to a probability distribution $\xvec_{i,t} \in \Delta_{\A_i}$, which is a stationary distribution of the matrix representing $\phi_{i,t}$.
%
This is crucial in order to implement the algorithm in a decentralized fashion and to provide convergence guarantees to constrained $\epsilon$-Phi-equilibria (see Theorem~\ref{th:learning_MCCCE}). 
%
All the distributions $\xvec_{i,t}$ jointly determine a correlated strategy $\zvec_t \in \Delta_{\A}$ at each round $t \in [T]$, defined as $\zvec_t := \otimes_{i\in \N} \, \xvec_{i,t}$, where $\otimes$ denotes the product among distributions; formally, $\zvec_t[\avec] := \prod_{i \in \N} \xvec_{i,t}[a_i]$ for all $\avec \in \A$.




Algorithm~\ref{alg:noregret} provides the following guarantees:
%
\begin{restatable}{theorem}{learning}\label{th:learning_MCCCE}
	Given an instance $I := (\Gamma,\Phi)$ satisfying Assumption~\ref{ass:cce}, after $T \in \mathbb{N}_{>0}$ rounds, Algorithm~\ref{alg:noregret} returns a correlated strategy $\bar\zvec_T \in \Delta_{\A}$ that is a constrained $\epsilon_T$-Phi-equilibrium with $\epsilon_T = O(\nicefrac{1}{\sqrt{T}})$.
	%
	Moreover, each round of Algorithm~\ref{alg:noregret} runs in polynomial time.
	%
	% Algorithm~\ref{alg:noregret}, after $T$ iterations, returns a Constrained $(\epsilon_T)$-equilibrium, where $\epsilon_T=O(T)$. Moreover the algorithm runs in polynomial time.
\end{restatable}
%
Let us remark that the crucial property which allows us to design Algorithm~\ref{alg:noregret} is that the sets $\Phi_i^\mcS$ of safe deviations do \emph{not} depend on players other than $i$.
%
Finally, from Theorem~\ref{th:learning_MCCCE}, the following result follows:
%
\begin{corollary}\label{cor:easy_main}
	In instances $I := (\Gamma,\Phi)$ satisfying Assumption~\ref{ass:cce}, a constrained $\epsilon$-Phi-equilibrium can be computed in time polynomial in the instance size and $\frac{1}{\epsilon}$ by means of a decentralized learning algorithm.
\end{corollary}



\subsection{Marginally-constrained CCE}\label{sec:easy_cce}



We conclude the section by introducing a particular (natural) notion of constrained $\epsilon$-Phi-equilibrium for which Assumption~\ref{ass:cce} is satisfied.
%
This is a constrained version of the classical CCE in cost-constrained normal-form games where a player's costs \emph{only} depend on the action of that player.
%
We call it \emph{marginally-constrained} $\epsilon$-CCE.
%
Formally, such an equilibrium is defined for games in which, for every player $i \in \N$, it holds $\cvec_i(\avec) = \cvec_i(\avec')$ for all $\avec, \avec' \in \A$ such that $a_i = a_i'$, and for the set $\Phi_{\textsc{CCE}}$ of CCE deviations that we have previously introduced in Section~\ref{sec:prelim_relations}.
%
%
%Assumption~\ref{ass:cce} holds in this natural setting. Consider the deviation set defined by $\Phi_{i,,\textnormal{CCE}}$ introduced in Section~\ref{sec:prelim} and the fact that the costs $\Cvec_i$ dependes only on the marginalization of the correlated strategy, \ie it exists a function $\tilde\Cvec^\prime:\Delta(\A_i)\to[-1,1]^m$ such that $\Cvec_i(\zvec)=\tilde\Cvec^\prime(\xvec_i)$ where $\xvec_i$ is the marginalized strategy of the $i$-th player, \ie $\xvec_i(a_i)=\sum_{\avec_i\in\A^{-i}}\zvec[a_i,\avec_{-i}]$. We can prove that under these conditions Assumption~\ref{ass:cce} holds.
%
%
Next, we prove that, with the definition above, Assumption~\ref{ass:cce} is satisfied.
%
\begin{restatable}{theorem}{marginal}\label{thm:marginal}
	For instances $I := (\Gamma, \Phi_{\textnormal{CCE}})$ such that $\cvec_i(\avec) = \cvec_i(\avec')$ for every player $i \in \N$ and action profiles $\avec, \avec' \in \A: a_i = a_i'$, Assumption~\ref{ass:cce} holds.
	%	
	%	If $\Phi_i=\Phi_{i,\textnormal{CCE}}$ for all $i\in[N]$ and the costs $\Cvec_i(\zvec)$ only depend on the marginalization $\xvec_i$ of $\zvec$ for the $i$-th player, then Assumption~\ref{ass:cce} holds.
\end{restatable}



Thanks to Theorem~\ref{thm:marginal}, we readily obtain the two following corollaries of Theorems~\ref{th:optimal_MCCCE}~and~\ref{th:optimal_MCCCE}.
%
\begin{corollary}
	The problem of computing a marginally-constrained (exact) CCE that maximizes a linear function $\ell: \Delta_{\A} \to \mathbb{R}$ can be solved in polynomial time.
	%
	%	Restricted to instances $I := (\Gamma, \Phi_{\textnormal{CCE}})$ such that $\cvec_i(\avec) = \cvec_i(\avec')$ for every $i \in \N$ and $\avec, \avec' \in \A: a_i = a_i'$, the problem \textsc{ApxCPE}$(1,0)$ admits a polynomial-time algorithm.
	%	
	%	There exists a polynomial time algorithm to compute an exact optimal Marginalized Constrained Coarse Correlated Equilibrium, for any linear function $\ell:\Delta(\A)\to[0,1]$.
\end{corollary}
%
\begin{corollary}
	A marginally-constrained $\epsilon$-CCE can be computed in time polynomial in the instance size and $\frac{1}{\epsilon}$ by means of a decentralized learning algorithm.
	%
	%
	% There exists a decoupled learning dynamics that converges to a Marginalized Constrained Coarse Correlated Equilibrium.
\end{corollary}


